T$^2$-Net: A Semi-supervised Deep Model for Turbulence Forecasting

Accurate air turbulence forecasting can help airlines avoid hazardous turbulence, guide the routes that keep passengers safe, maximize efficiency, and reduce costs. Traditional turbulence forecasting approaches heavily rely on painstakingly customized turbulence indexes, which are less effective in dynamic and complex weather conditions. The recent availability of high-resolution weather data and turbulence records allows more accurate forecasting of the turbulence in a data-driven way. However, it is a non-trivial task for developing a machine learning based turbulence forecasting system due to two challenges: (1) Complex spatio-temporal correlations, turbulence is caused by air movement with complex spatio-temporal patterns, (2) Label scarcity, very limited turbulence labels can be obtained. To this end, in this paper, we develop a unified semi-supervised framework, T$^2$-Net, to address the above challenges. Specifically, we first build an encoder-decoder paradigm based on the convolutional LSTM to model the spatio-temporal correlations. Then, to tackle the label scarcity problem, we propose a novel Dual Label Guessing method to take advantage of massive unlabeled turbulence data. It integrates complementary signals from the main Turbulence Forecasting task and the auxiliary Turbulence Detection task to generate pseudo-labels, which are dynamically utilized as additional training data. Finally, extensive experimental results on a real-world turbulence dataset validate the superiority of our method on turbulence forecasting.

==> ICDM20 2/conclusion.tex <==
\section{Conclusion}
In this paper, we developed a data-driven framework for turbulence forecasting. Specifically, we first built an encoder-decoder paradigm based on ConvLSTM to model the spatio-temporal correlations. Then, to address the label scarcity issue, we proposed a novel {Dual Label Guessing} method, which integrated complementary signals from the main task of {\tb{T}}urbulence Forecasting and the auxiliary task of {\tb{T}}urbulence Detection to generate pseudo-labels. 
% These pseudo-labels were further reweighted by the heuristic {Label Quality Detector} according to their reliability. 
Finally, we conducted extensive experiments on a real-world dataset which showed that the proposed approach can greatly alleviate the problem of spatio-temporal correlation modeling as well as label scarcity on turbulence forecasting.



==> ICDM20 2/experiments.tex <==
\section{Experiments}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{figure*}
% \abovecaptionskip
% \belowcaptionskip
% \setlength{\belowcaptionskip}{-10pt}
\centering
% \subfigure[Accuracy]{\label{a1}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/o1-.pdf}}
% \subfigure[Weighted-Precision]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/o2-.pdf}}
% \subfigure[Weighted-Recall]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/o3-.pdf}} 
% \subfigure[Weighted-F1]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=5.1cm]{./figures/o4--.pdf}}  
\subfigure[Accuracy]{\label{a1}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/e1.pdf}}
\subfigure[Weighted-Precision]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/e2.pdf}}
\subfigure[Weighted-Recall]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=3.9cm]{./figures/e3.pdf}} 
\subfigure[Weighted-F1]{\label{a2}\includegraphics[trim=0 20 0 0, clip, width=4.7cm]{./figures/e4.pdf}}  
% \vspace{-4mm}
\caption{Performance comparison of different forecasting lengths.}\label{hours}
\vspace{-6mm}
\end{figure*}
In this section, we first introduce the data and settings of our experiments. 
Then we evaluate the performances of the proposed forecasting model on different forecasting lengths compared with several state-of-the-art baselines. 
Lastly, we show the parameter sensitivity analysis.
% as well as the complexity analysis.
% Finally we show some case studies of our model applying to turbulence forecasting.
\subsection{Experimental Settings}
\noindent\tb{Data Preprocessing:} All the data we use in the experiment are publicly available. 
% All the data we use in the experiment are collected online. 
We first obtain
% 7 days of weather data (from 20190601 to 20190607) 
 30 days of weather data (from 20190601 to 20190630) 
from National Oceanic and Atmospheric Administration (NOAA) \footnote{ftp://nomads.ncdc.noaa.gov/RUC/13km/201906/}, then obtain 30 days of turbulence report data (the same period as the weather data) from Iowa Environmental Mesonet (IEM) \footnote{http://mesonet.agron.iastate.edu/request/gis/pireps.php}. 
The weather data is generated hourly on a 13-km (8-mile) resolution horizontal grid, with $451\times337$ grids in total, representing the North American region. 
In vertical direction, there are 36 different geopotential heights.
% Figure \ref{visualization} shows four visualization examples of the raw data, e.g., the v-component of wind, temperature, vertical velocity and relative humidity at one certain isobaric surface (warmer color indicates higher value).
We treat the whole data as a \ti{$451\times337\times36$} cube and use a sliding window of size $10\times10\times5$ to generate the hourly \ti{feature cubes} (each grid contains the raw weather features and the turbulence indexes). 
For the turbulence report, each report contains the coordinate, geopotential height, time, and level of the turbulence, and we use the same way to generate the hourly \ti{label cubes} (each grid contains the turbulence level). 
We filter out the cubes NOT in the ``cruising altitude'' (31000 to 38000 feet) since most pilot reports are recorded among these heights. 
% \lyc{the number of height after filtering?}.
Finally, we use a sliding window of $n+p$ hours, adopt the first $n$ hours' feature cubes as the input sequence and the next $p$ hours' label cubes as the output sequence to generate the training data. 
In experiments, we investigated different $n$ and $p$, specifically, $n=p=\{3,6,12,24\}$.
% Finally we use a sliding window of 14 hours in each day, adopt the first 7 hours' feature cubes as the input sequence and the next 7 hours' label cubes as the output sequence to generate the training data. 
We further randomly split the data into training/validation/testing set with the ratio of {6:2:2}.

% \begin{figure*}[htbp]
% \centering
% \begin{minipage}[t]{0.235\textwidth}
% \centering
% \includegraphics[width=4cm]{./figures/visual-1.pdf}
% % \caption{World Map}
% \end{minipage}
% \begin{minipage}[t]{0.235\textwidth}
% \centering
% \includegraphics[width=4cm]{./figures/visual-2.pdf}
% % \caption{Concrete and Constructions}
% \end{minipage}
% \begin{minipage}[t]{0.235\textwidth}
% \centering
% \includegraphics[width=4cm]{./figures/visual-1.pdf}
% % \caption{World Map}
% \end{minipage}
% \begin{minipage}[t]{0.235\textwidth}
% \centering
% \includegraphics[width=4cm]{./figures/visual-2.pdf}
% % \caption{Concrete and Constructions}
% \end{minipage}
% \caption{Visualization of the weather data.}
% \label{visualization}
% \end{figure*}

\begin{table}
\small
\caption{Overall performance of $\text{T}^{2}$-Net and baselines.}
	\centering
	\begin{tabular}{c|c|c|c|c}
		\hline
		\hline
		\multirow{2}*{Method} & \multirow{2}*{Accuracy} & \multicolumn{3}{c}{Weighted}   \\
		\cline{3-5}
		~ & ~  & P &R & F1 \\
		\hline
		\hline 
		 TBI (Turbulence indexes)  &0.428  &0.368  &0.428 &0.382  \\ %\cline{2-9}
		 Multinomial LR  &0.434  &0.355  &0.434 &0.385  \\ %\cline{2-9}
		 MLP (3-layers) &0.449  &0.393  &0.449 &0.355  \\  %\cline{2-9}
		 GBDT (100 trees) &0.440  &0.370 &0.440 &0.341 \\  %\cline{2-9}
		  Attentional LSTM &0.489 & 0.378 &0.489 & 0.426 \\ %\cline{2-9}
		  CNN (kernel size=3) &0.491 & 0.437 &0.491 & 0.370 \\  %\cline{2-9}
		  % ~ &ConvLSTM (N-to-N) & &   & &  &  & &  \\  %\cline{2-9}
		  % ~ &\textbf{ConvLSTM+pseudo-labeling} & &   & &  &  & &  \\ 
		% \hline
			% LSTM (Seq2seq)  &  &   & &  &  & &  \\  %\cline{2-9}
		 ConvLSTM &0.571   &0.548  &0.581 &0.518  \\ %\cline{2-9}
		 Hetero-ConvLSTM &0.580   &0.536  &0.580 &0.520  \\ %\cline{2-9}
		\hline
% 		 AQI (Air quality inference) &0.589   &0.528  &0.592 &0.529  \\  %\cline{2-9}
		 Pseudo-labeling &0.591   &0.536  &0.600 &0.536  \\
		 Mixmatch &0.600   &0.546  &0.580 &0.540  \\
		\hline
		% \multicolumn{2}{|c|}{$\text{T}^{2}$-Net(All)} & & ~ &   & &  &  & \\
% 		 $\text{T}^{2}$-Net &\tb{0.631} & \tb{0.553} &\tb{0.621}  &\tb{0.552} \\
		 $\text{T}^{2}$-Net &\tb{0.623} & \tb{0.551} &\tb{0.614}  &\tb{0.548} \\
		\hline
		\hline
	\end{tabular}
\label{overall}
\vspace{-6mm}
\end{table}

\noindent\tb{Evaluation Metrics: }
% As mentioned in Section 2, we formulate the turbulence forecasting problem as a sequence to sequence multi-class classification problem. 
We adopt several standard multi-class classification metrics to evaluate all the models: (1) Accuracy, (2) Weighted-Precision, (3) Weighted-Recall, (4) Weighted-F1. 
% Accuracy reflects the ratio of the correctly classified in the test set. 
% Recall expresses the ability to find all relevant instances of a class; precision expresses the proportion of the samples a model predicted relevant actually were relevant. 
% F1 score is the harmonic mean of precision and recall. 
% \ti{Weighted} indicates the averaging method used for multi-class problem. 
% which take class imbalance into account. 
% For instance, Weighted-F1 first calculate the F1 score of all the classes and then return the average F1 weighted by support (the number of true instances for each class). 
We calculate these metrics by averaging them throughout all the labeled grids in different time steps and skip the grids labeled with ``unknown''.

% \noindent\tb{Evaluation Metrics: }As mentioned in Section 2, we formulate the turbulence forecasting problem as a sequence to sequence multi-class classification problem. We adopt several standard multi-class classification metrics to evaluate all the models: (1) Accuracy, (2) Macro-Precision, (3) Macro-Recall, (4) Macro-F1, (5) Weighted-Precision, (6) Weighted-Recall (7) Weighted-F1. Accuracy reflects the ratio of the correctly classified in the test set. Recall expresses the ability to find all relevant instances of a class, precision expresses the proportion of the samples a model says was relevant actually were relevant. F1 score is the harmonic mean of precision and recall. \ti{Macro} and \ti{Weighted} are two averaging methods for multi-class. \ti{Macro} simply average all classes while \ti{Weighted} account for class imbalance and find their average weighted by support (the number of true instances for each class). We calculate these metrics by averaging them throughout all the labeled grids in different time steps and mask the grids labeled with `unknown'.
\noindent\tb{Parameter Configuration: }For our model and all the baseline methods, we obtain the optimal parameters on the validation set using early stopping. 
% The key hyperparameters of \model{} include $\beta$, $T_1$, $T_2$, $T$, $\lambda$, $\gamma$. 
For TFN, we adopt 1-layer ConvLSTM with $3\times3\times3$ kernel for both encoder and decoder, using Sigmoid as activation function. For TDN, we adopt 3-layer CNN with  $3\times3\times3$, $3\times3\times3$ and $5\times5\times3$ kernels respectively, using Relu as inner activation function.
The optimal hyperparameters of the rest part are $\beta=0.6, T_1=5, T_2=15, T=0.5, \lambda=0.4$.
% \gamma =2$.

\noindent\tb{Baseline Methods: }To systematically investigate the performance of modern machine learning methods on turbulence forecasting, we compare our proposed \model{} with 3 categories of baselines. (1) \ti{Tubulence indexes} (\tb{TBI}) \cite{sharman2006integrated}, an integrated approach which combines multiple turbulence indexes to forecast turbulence. (2) \ti{Supervised learning methods}: a number of supervised machine learning methods are examined: Multinomial Logistic Regression (\tb{Multinomial LR}), Multi-layer Perceptron (\tb{MLP}), Gradient Boosting Decision Tree (\tb{GBDT}) \cite{friedman2001greedy}, \tb{Attentional LSTM}, Convolutional Neural Network (\tb{CNN}), \tb{ConvLSTM} \cite{xingjian2015convolutional} and \tb{Hetero-ConvLSTM} \cite{yuan2018hetero}. 
% Among these models, Multinomial LR, MLP and GBDT are normal classification models, while Attentional LSTM, CNN, ConvLSTM and Hetero-ConvLSTM introduce complex spatial/temporal correlation. Attentional LSTM and CNN only models temporal and spatial correlation respectively, ConvLSTM extends LSTM .
% For the reason of space limits, we omit the detail of these methods.
We test all these methods using the same base features as our model, i.e., the 6 raw weather features and 6 turbulence indexes. (3) \ti{Semi-supervised learning (SSL) methods}: we also compare with several state-of-the-art semi-supervised learning methods since abundant unlabeled data exists in the turbulence forecasting task and \model{} is also semi-supervised. \tb{Pseudo-labeling} \cite{lee2013pseudo}, a simple yet effective SSL method which retrains the model with pseudo-labels predicted by the model itself. 
% Air Quality Inference (\tb{AQI}) model \cite{hsieh2015inferring}, a graph-based semi-supervised learning method for inferring air quality of arbitrary location using very sparse monitoring data.
\tb{Mixmatch} \cite{berthelot2019mixmatch}, a recent holistic approach which unifies several dominant SSL methods and achieves state-of-the-art results on 4 benchmark datasets. To ensure a fair comparison, we apply the same base model (ConvLSTM) for these SSL methods.

% \begin{figure*}[htbp]
% \centering
% % \abovecaptionskip
% % \belowcaptionskip
% % \setlength{\belowcaptionskip}{-10pt}
% % \subfigure[Accuracy]{\label{a1}\includegraphics[width=4.3cm]{./figures/acc-hours1.pdf}}
% \subfigure[Precision]{\label{a2}\includegraphics[trim=0 20 0 30, clip, width=4.4cm]{./figures/s1-.pdf}}
% \subfigure[Recall]{\label{a2}\includegraphics[trim=0 20 0 30, clip, width=4.4cm]{./figures/s2-.pdf}} 
% \subfigure[F1]{\label{a2}\includegraphics[trim=0 20 0 10, clip, width=6.4cm]{./figures/s3-.pdf}} 
% % \vspace{-4mm}
% \caption{Performance comparison on the minority class (Level: severe).}\label{minority}
% % \vspace{-6mm}
% \end{figure*}

\begin{figure*}[htbp]
\centering
% \abovecaptionskip
% \belowcaptionskip
% \setlength{\belowcaptionskip}{-10pt}
% \subfigure[$\beta$]{\label{a1}\includegraphics[trim=0 40 0 10, clip, width=4.1cm]{./figures/p1.pdf}}
% \subfigure[T]{\label{a2}\includegraphics[trim=0 40 0 10, clip, width=4.1cm]{./figures/p2.pdf}}
% \subfigure[$\lambda$]{\label{a2}\includegraphics[trim=0 40 0 10, clip, width=4.1cm]{./figures/p3.pdf}} 
% \subfigure[$\gamma$]{\label{a2}\includegraphics[trim=0 40 0 10, clip, width=5.51cm]{./figures/p4.pdf}}  
\subfigure[$\beta$]{\label{a1}\includegraphics[ width=4.8cm]{./figures/sensitivity1-.pdf}}
% \hspace{-5mm}
\subfigure[T]{\label{a2}\includegraphics[ width=4.8cm]{./figures/sensitivity2-.pdf}}
% \hspace{-5mm}
\subfigure[$\lambda$]{\label{a2}\includegraphics[ width=4.8cm]{./figures/sensitivity3-.pdf}} 
% \hspace{-5mm}
% \subfigure[$\gamma$]{\label{a2}\includegraphics[ width=4.8cm]{./figures/sensitivity4-.pdf}} 
% \hspace{-10mm} 
% \vspace{-4mm}
\caption{Parameter sensitivity analysis.}\label{parameter}
\vspace{-6mm}
\end{figure*}
\subsection{Overall Results on Turbulence Forecasting}
We first present the overall performance of all baselines and \model{} when $n=p=6$. 
The results are presented in Table \ref{overall}. 
MLP and GBDT perform better than TBI and Multinomial LR because they integrate nonlinearity. 
By taking temporal correlation and spatial correlation into consideration, Attentional LSTM and CNN achieve better accuracy than those not. 
ConvLSTM further improves the performance because of modeling spatial and temporal correlation simultaneously. 
Hetero-ConvLSTM achieves the best accuracy and Weighted F1 among supervised methods for it predicts based on an ensemble of multiple ConvLSTMs of different geographical areas. 
However, Hetero-ConvLSTM has an efficiency issue for training many ConvLSTMs at the same time.
For the semi-supervised learning baselines, all of them beat the supervised methods, verifying the practicability of taking advantage of unlabeled data. 
Among them, Mixmatch achieves the best accuracy, Weighted F1, Weighted Precision, and thus proves that \ti{soft pseudo-label} is better than \ti{hard pseudo-label}.  
\model{} achieves the best performance with the highest Accuracy, Weighted Precision/Recall/F1. 
This indicates that on turbulence forecasting task, \model{} has superior ability to model the complex spatio-temporal relation as well as utilizing the abundant unlabeled data to enhance training.
% \lyc{results on other lengths not included}

We also report the overall performance of \model{} and several representative baselines (ConvLSTM, Hetero-ConvLSTM, and Mixmatch) for different forecasting lengths ($n=p=3,6,12,24$). 
As shown in Figure \ref{hours}, we can observe that \model{} achieves the best performance on different time lengths. 
However, an interesting phenomenon brought to our attention is that when $n,p$ increases ($>$6), there is a drop in performance for all the baseline models and \model. 
We attribute this to the increased complexity and ``gradient vanishing'' problem in long-sequence prediction. 
However, performance on $n,p=6$ is better than $n,p=3$, this is because the model benefits more from the increased input feature length when the time length changes from 3 to 6.



% \begin{table}
% \caption{Overall performance of $\text{T}^{2}$-Net and baselines.}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c}
% 		\hline
% 		\hline
% 		~ & \multirow{2}*{Accuracy} & \multicolumn{3}{c}{Weighted}   \\
% 		\cline{3-5}
% 		~ & ~  & P  &R & F1 \\
% 		\hline
% 		\hline 
% 		 TBI (Turbulence indexes)  &0.4289  &0.3682  &0.4289 &0.3825  \\ %\cline{2-9}
% 		 Multinomial LR  &0.4349  &0.3553  &0.4348 &0.3850  \\ %\cline{2-9}
% 		 MLP (3-layers) &0.4493  &0.3932  &0.4493 &0.3550  \\  %\cline{2-9}
% 		 GBDT (100 trees) &0.4408  &0.3700 &0.4407 &0.3414 \\  %\cline{2-9}
% 		  Attentional LSTM &0.4892 & 0.3785 &0.4892 & 0.4267 \\ %\cline{2-9}
% 		  CNN (kernel size=3) &0.4912 & 0.4376 &0.4912 & 0.3709 \\  %\cline{2-9}
% 		  % ~ &ConvLSTM (N-to-N) & &   & &  &  & &  \\  %\cline{2-9}
% 		  % ~ &\textbf{ConvLSTM+pseudo-labeling} & &   & &  &  & &  \\ 
% 		% \hline
% 			% LSTM (Seq2seq)  &  &   & &  &  & &  \\  %\cline{2-9}
% 		 ConvLSTM &0.5717   &0.5485  &0.5816 &0.5182  \\ %\cline{2-9}
% 		 Hetero-ConvLSTM &0.5809   &0.5361  &0.5808 &0.5144  \\ %\cline{2-9}
% 		\hline
% 		 AQI (Air quality inference) &0.5890   &0.5281  &0.5928 &0.5294  \\  %\cline{2-9}
% 		 Pseudo-labeling &0.5912   &0.5362  &0.6008 &0.5364  \\
% 		 Mixmatch &0.6009   &0.5460  &0.5809 &0.5279  \\
% 		\hline
% 		% \multicolumn{2}{|c|}{$\text{T}^{2}$-Net(All)} & & ~ &   & &  &  & \\
% 		 $\text{T}^{2}$-Net (All) &\tb{0.6310} & \tb{0.5536} &\tb{0.6210}  &\tb{0.5527} \\
% 		\hline
% 		\hline
% 	\end{tabular}
% \label{overall}
% \end{table}
% \begin{table*}
% \caption{Overall performance of $\text{T}^{2}$-Net and baselines.}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c|c|c}
% 		\hline
% 		\hline
% 		~ & \multirow{2}*{Accuracy} & \multicolumn{3}{c|}{Macro} & \multicolumn{3}{c}{Weighted}   \\
% 		\cline{3-8}
% 		~ & ~ & Precision  &Recall & F1 & Precision  &Recall & F1 \\
% 		\hline
% 		\hline 
% 		 TBI (Turbulence indexes)  &0.4289 &0.1925   &0.2074 &0.1886  &0.3682  &0.4289 &0.3825  \\ %\cline{2-9}
% 		 Multinomial LR  &0.4349 &0.1792   &0.2087 &0.1884  &0.3553  &0.4348 &0.3850  \\ %\cline{2-9}
% 		 MLP (3-layers) &0.4493 &0.2283   &0.2031 &0.1705  &0.3932  &0.4493 &0.3550  \\  %\cline{2-9}
% 		 GBDT (100 trees) &0.4408 &0.2109  &0.1977 &0.1617  &0.3700 &0.4407 &0.3414 \\  %\cline{2-9}
% 		  Attentional LSTM &0.4892 &0.1876   &0.2409 & 0.2108 & 0.3785 &0.4892 & 0.4267 \\ %\cline{2-9}
% 		  CNN (kernel size=3) &0.4912 &0.2501   &0.2109 & 0.1664 & 0.4376 &0.4912 & 0.3709 \\  %\cline{2-9}
% 		  % ~ &ConvLSTM (N-to-N) & &   & &  &  & &  \\  %\cline{2-9}
% 		  % ~ &\textbf{ConvLSTM+pseudo-labeling} & &   & &  &  & &  \\ 
% 		% \hline
% 			% LSTM (Seq2seq)  &  &   & &  &  & &  \\  %\cline{2-9}
% 		 ConvLSTM &0.5717  &0.2660   &0.2712 &0.2521  &0.5485  &0.5816 &0.5182  \\ %\cline{2-9}
% 		 Hetero-ConvLSTM &0.5809  & 0.2727  &0.2734 &0.2526  &0.5361  &0.5808 &0.5144  \\ %\cline{2-9}
% 		\hline
% 		 AQI (Air quality inference) &0.5890  & 0.2933  &0.2914 &0.2701  &0.5281  &0.5928 &0.5294  \\  %\cline{2-9}
% 		 Pseudo-labeling &0.5912  & 0.2927  &0.2834 &0.2626  &0.5362  &0.6008 &0.5364  \\
% 		 Mixmatch &0.6009  & 0.2811  &0.2715 &0.2677  &0.5460  &0.5809 &0.5279  \\
% 		\hline
% 		% \multicolumn{2}{|c|}{$\text{T}^{2}$-Net(All)} & & ~ &   & &  &  & \\
% 		 $\text{T}^{2}$-Net (All) &\tb{0.6310} &\tb{0.3070} &\tb{0.3050}   &\tb{0.2710} & \tb{0.5536} &\tb{0.6210}  &\tb{0.5527} \\
% 		\hline
% 		\hline
% 	\end{tabular}
% \label{overall}
% \end{table*}



% \begin{figure}
% % \abovecaptionskip
% % \belowcaptionskip
% % \setlength{\belowcaptionskip}{-10pt}
% \subfigure[Accuracy]{\label{a1}\includegraphics[width=4cm]{./figures/acc-hours1.pdf}}
% \subfigure[Weighted-Precision]{\label{a2}\includegraphics[width=4cm]{./figures/acc-hours1.pdf}}
% \subfigure[Weighted-Recall]{\label{a2}\includegraphics[width=4cm]{./figures/acc-hours1.pdf}} 
% \subfigure[Weighted-F1]{\label{a2}\includegraphics[width=4cm]{./figures/acc-hours1.pdf}}  
% \vspace{-2mm}
% \caption{Performance comparison of different forecasting length.}\label{hours}
% % \vspace{-6mm}
% \end{figure}

% \subsection{Results on Extreme Turbulence Conditions}
% \subsection{Results on Minority Class}
% We further evaluate the performance of turbulence forecasting on the minority class, i.e., turbulence level ``severe''. 
% %Figure \ref{minority} presents the results on The performance on level ``severe'' is critical for turbulence forecasting since it is level ``severe'' that 
% Severe turbulence causes most of the in-flight injuries and aircraft damage, thus a higher precision/recall on ``severe'' is the most critical to airline safety. 
% As shown in Figure \ref{minority}, our \model{} outperforms all baselines significantly, on all metrics and all time lengths. 
% Specifically, when $n=p=6$, it exceeds the second place more than  34\% on Precision, 33\% on Recall and 36\% on F1 respectively. 
% This validates that our hybrid loss function of Focal Loss and Weighted-L2 can greatly alleviate the issue of label imbalance, thus making \model{} a more practical solution for turbulence forecasting. 

% \begin{table}
% % \small
% \normalsize
% \caption{Training and Forecasting Efficiency}
% % \vspace{-2mm}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% % 		\hline
% % 		Code&/NEG&/LGT&/MOD&/SEV\\
% 		\hline
% 		Computing resource&Training&Forecasting\\
% 		\hline
% 		GeForce GTX 1080 Ti& 640s&5.8s \\
% 		\hline
% 	\end{tabular}
% \label{efficiency}
% \end{table}
\subsection{Parameter Sensitivity Analysis}
Figure \ref{parameter} presents the sensitivity analysis of the key parameters of our Dual Label Guessing
and loss function, i.e., $\beta, T,$ and $\lambda$. 
We obtained the sensitivity curve of each parameter by fixing the rest using their optimal values. 
We can observe that the best performance is achieved when $\beta=0.6$ , this indicates TFN is more important to the final result. 
Besides, $\lambda=0.4$ achieves the best results indicating that there is a trade-off of utilizing the unlabeled data.
We can also observe that the performance is relatively stable as the parameters change, thus proves the robustness of \model.

% \subsection{Deployment Consideration}
% Our framework presents a data-driven solution for 3/6/12/24 hours of turbulence forecasting. 
% Currently, the experimental results are carried out on 30 days meteorological data of the North America area. 
% We can still use this data source for different countries since deep models have strong generalization power to learn turbulence patterns that can generalize among different geographical regions. 
% However, to deploy a realtime system for airline companies or the public, a major challenge is the efficiency issue. 
% The time of feature extraction is negligible since it can be computed in parallel.
% Table \ref{efficiency} shows the average training and forecasting time of \model{} for 10,000 samples on a single GeForce GTX 1080 Ti. 
% The forecasting length is 6 hours, the forecasting area is $10\times10\times5$. 
% It only takes about 11 minutes to train and 5.8s for forecasting. 
% To cover the North America area, we only need to forecast 6,000 samples of shape $10\times10\times5$, and the efficiency can be further improved with more GPUs, thus \model{} is feasible for large-scale real-time turbulence forecasting.

% % \begin{figure*}[htbp]
% % \centering
% % \begin{minipage}[t]{0.235\textwidth}
% % \centering
% % \includegraphics[width=4cm]{./figures/acc-hours2.pdf}
% % % \caption{World Map}
% % \end{minipage}
% % \begin{minipage}[t]{0.235\textwidth}
% % \centering
% % \includegraphics[width=4cm]{./figures/acc-hours2.pdf}
% % % \caption{Concrete and Constructions}
% % \end{minipage}
% % \begin{minipage}[t]{0.235\textwidth}
% % \centering
% % \includegraphics[width=4cm]{./figures/acc-hours2.pdf}
% % % \caption{World Map}
% % \end{minipage}
% % \begin{minipage}[t]{0.235\textwidth}
% % \centering
% % \includegraphics[width=4cm]{./figures/acc-hours2.pdf}
% % % \caption{Concrete and Constructions}
% % \end{minipage}
% % \caption{Performance of different forecasting length.}
% % \label{visualization}
% % \end{figure*}



% % \subsection{Case Studies and Deployment}

% % \begin{table*}
% % \caption{Overall performance of $\text{T}^{2}$-Net and baselines.}
% % 	\centering
% % 	\begin{tabular}{c|c|c|c|c|c|c|c}
% % 		\hline
% % 		\hline
% % 		~ & \multirow{2}*{Accuracy} & \multicolumn{3}{c|}{Macro} & \multicolumn{3}{c}{Weighted}   \\
% % 		\cline{3-8}
% % 		~ & ~ & Precision  &Recall & F1 & Precision  &Recall & F1 \\
% % 		\hline
% % 		\hline 
% % 		 TBI (7 turbulence indexes)  & &   & &  &  & &  \\ %\cline{2-9}
% % 		 LR (Multinomial)  & &   & &  &  & &  \\ %\cline{2-9}
% % 		 MLP (3-layers) & &   & &  &  & &  \\  %\cline{2-9}
% % 		 GBDT (100 trees) & &   & &  &  & &  \\  %\cline{2-9}
% % 		  LSTM & &   & &  &  & &  \\ %\cline{2-9}
% % 		  CNN (kernel size=3) & &   & &  &  & &  \\  %\cline{2-9}
% % 		  % ~ &ConvLSTM (N-to-N) & &   & &  &  & &  \\  %\cline{2-9}
% % 		  % ~ &\textbf{ConvLSTM+pseudo-labeling} & &   & &  &  & &  \\ 
% % 		% \hline
% % 			% LSTM (Seq2seq)  &  &   & &  &  & &  \\  %\cline{2-9}
% % 		 AQI &  &   & &  &  & &  \\  %\cline{2-9}
% % 		 ConvLSTM &  &   & &  &  & &  \\ %\cline{2-9}
% % 		 Hetero-ConvLSTM &  &   & &  &  & &  \\ %\cline{2-9}
% % 		\hline
% % 		 Pseudo-labeling &  &   & &  &  & &  \\
% % 		 Mixmatch &  &   & &  &  & &  \\
% % 		\hline
% % 		% \multicolumn{2}{|c|}{$\text{T}^{2}$-Net(All)} & & ~ &   & &  &  & \\
% % 		 $\text{T}^{2}$-Net (All) & & ~ &   & &  &  & \\
% % 		\hline
% % 		\hline
% % 	\end{tabular}
% % \end{table*}


% % \begin{table*}
% % \caption{Overall performance of $\text{T}^{2}$-Net and baselines.}
% % 	\centering
% % 	\begin{tabular}{c|c|c|c|c|c|c|c|c}
% % 		\hline
% % 		\hline
% % 		\multicolumn{2}{c|}{~} & \multirow{2}*{Accuracy} & \multicolumn{3}{c|}{Macro} & \multicolumn{3}{c}{Weighted}   \\
% % 		\cline{4-9}
% % 		\multicolumn{2}{c|}{~} & ~ & Precision  &Recall & F1 & Precision  &Recall & F1 \\
% % 		\hline
% % 		\hline 
% % 		\multirow{5}*{Tubulence index based models } &LR (Multinomial)  & &   & &  &  & &  \\ %\cline{2-9}
% % 		 ~&MLP (3-layers)& &   & &  &  & &  \\  %\cline{2-9}
% % 		 ~&GBDT (100 trees)& &   & &  &  & &  \\  %\cline{2-9}
% % 		  ~&LSTM (N-to-N) & &   & &  &  & &  \\ %\cline{2-9}
% % 		  ~ &CNN (kernel size=3)& &   & &  &  & &  \\  %\cline{2-9}
% % 		  ~ &ConvLSTM (N-to-N) & &   & &  &  & &  \\  %\cline{2-9}
% % 		  ~ &\textbf{ConvLSTM+pseudo-labeling} & &   & &  &  & &  \\ 
% % 		\hline
% % 		 \multirow{4}*{Machine learning models} &LSTM (Seq2seq)  &  &   & &  &  & &  \\  %\cline{2-9}
% % 		 ~&ConvLSTM (Seq2seq) &  &   & &  &  & &  \\  %\cline{2-9}
% % 		  ~&AQI &  &   & &  &  & &  \\ %\cline{2-9}
% % 		  ~ &\textbf{ConvLSTM+pseudo-labeling} &  &   & &  &  & &  \\
% % 		\hline
% % 		% \multicolumn{2}{|c|}{$\text{T}^{2}$-Net(All)} & & ~ &   & &  &  & \\
% % 		Heterogeneous Models& $\text{T}^{2}$-Net (All) & & ~ &   & &  &  & \\
% % 		\hline
% % 		\hline
% % 	\end{tabular}
% % \end{table*}



==> ICDM20 2/figures/methodology.tex <==
\section{Methodology}
% \lyc{need to highlight the technical contribution, now it looks like a combination of existing methods}
In this section, we introduce the details of our turbulence forecasting framework, \model. As shown in Figure \ref{framework}, \model mainly consists of a \ti{\large{\tb{T}}urbulence Forecasting Network} (\tb{T}FN), a \ti{\large{\tb{T}}urbulence Detection Network} (\tb{T}DN). 
% and a \ti{Dual Label Guessing} module. 
TFN serves for the main task, i.e., forecasting task, while
% forecasting the turbulence conditions at next few hours. 
% TDN serves for the detection task, i.e., an auxiliary task providing clues for accurate pseudo-label generation.
TDN serves for the auxiliary task, i.e., detection task, which provides complementary semi-supervised signals for the main task. Based on the predictions of TFN and TDN, a novel \ti{\tb{Dual Label Guessing}} approach is proposed to fuse these two sources of information to generate more robust pseudo-labels as additional training data. In order to minimize the effect of "bad" pseudo-labels, the grids tagged with pseudo-labels are reweighted by our heuristic \ti{\tb{Label Quality Detector}} (LQD) based on the quality scores, and added into training loop dynamically. 
% To further improve the label quality, a novel Local Consistency Regularization is imposed at the output of TFN.
\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-7pt}
\centering
\includegraphics[width=0.48\textwidth]{./figures/framework2.pdf}
\vspace{-0.6cm}
\caption{Overview of \model.}
\label{framework}
\vspace{-0.1cm}
\end{figure}
\subsection{Turbulence Forecasting Network}
% TFN employs the architecture of ConvLSTM\cite{xingjian2015convolutional} to model the spatiotemporal correlations among the grids. 
TFN is designed on top of the basic ConvLSTM \cite{xingjian2015convolutional} architecture to model the complex spatiotemporal correlations among different spatial grids. ConvLSTM is a variation of LSTM to handle spatiotemporal prediction tasks. It extends basic LSTM cell by replacing the fully connected layer with convolution operatoration in the internal transitions.
The key equations of ConvLSTM are shown in (3)\text{-}(7) below, where $X_t, o_t,H_t$ are the input, output and hidden vectors respectively, `$\circledast $' denotes the \ti{3D-convolution} operator and `$\circ$' denotes the Hadamard product:
% \begin{large}
\begin{equation}
i_t=\sigma(W_{xi}\circledast X_t+W_{hi}\circledast H_{t-1}+W_{ci}\circ C_{t-1}+b_i)
\end{equation}
\begin{equation}
f_t = \sigma(W_{xf}\circledast X_t+W_{hf}\circledast H_{t-1}+W_{cf}\circ C_{t-1}+b_f)
\end{equation}
\begin{equation}
C_t = f_t\circ C_{t-1} +i_t\circ tanh(W_{xc}\circledast X_t+W_{hc}\circledast H_{t-1}+b_c)
\end{equation}
\begin{equation}
o_t = \sigma(W_{xo}\circledast X_t+W_{ho}\circledast H_{t-1}+W_{co}\circ C_t+b_o)
\end{equation}
\begin{equation}
H_t =o_t\circ tanh(C_t)
\end{equation}
% \end{large}
% \begin{equation}
% \begin{aligned}
%     &i_t=\sigma(W_{xi}*X_t+W_{hi}*H_{t-1}+W_{ci}\circ C_{t-1}+b_i)\\
%    & f_t = \sigma(W_{xf}*X_t+W_{hf}*H_{t-1}+W_{cf}\circ C_{t-1}+b_f)\\
%     &C_t = f_t\circ C_{t-1} +i_t\circ tanh(W_{xc}*X_t+W_{hc}*H_{t-1}+b_c)\\
%     &o_t = \sigma(W_{xo}*X_t+W_{ho}*H_{t-1}+W_{co}\circ C_t+b_o)\\
%    & H_t =o_t\circ tanh(C_t)
% \end{aligned}
% \end{equation}
As shown in the bottom part of Figure \ref{framework}, TFN consists of two ConvLSTMs, serving as the encoder and decoder respectively. The encoder takes a squence of 4D tensors as input, i.e., $X_1,X_2,...,X_n \in \mathbb{R}^{\mc{L\times W\times H \times C}}$, the historical turbulence feature cubes of time slot $1,...,n$. $\mc{L\times W\times H} $ is the shape of a grid-based 3D region and $\mc{C}$ is the number of channels/features for each grid. The decoder takes the last hidden state of the encoder as the initial hidden state, and uses \ti{teacher forcing} \cite{goodfellow2016deep} (use previous ground truth $Y_{j-1}$ as the next input to the decoder) to generate a sequence of features corresponding to the forecasting time stamps $n+1,...,n+p$. The decoder's outputs are then fed into to a $\text{Conv}1\times 1$ block followed with a Softmax layer to produce the forecasted turbulence conditions $P_{n+1},P_{n+2},...,P_{n+p} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
% The decoder's outputs are then concatenated with the forecasted turbulence features at multiple forecasting time stamps, $X'_{n+1},X'_{n+2},..., X'_{n+p} \in \mathbb{R}^{\mc{L\times W\times H  \times C}}$, and fed into to a $Conv1\times 1$ block followed with a $softmax$ layer to produce the forecasted turbulence conditions $P_{n+1},P_{n+2},...,P_{n+p} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
The process of TFN can be summarized in equation (8)-(10):
% \begin{normalsize}
\begin{large}
\begin{equation}
h_i^{enc},o_i^{enc} = \text{ConvLSTM}^{enc}(X_{i},h_{i-1}^{enc}), i\in[1,n]
\end{equation}
\begin{equation}
h_j^{dec},o_j^{dec} = \text{ConvLSTM}^{dec}(Y_{j-1}, h_{j-1}^{dec}),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation}
\begin{equation}
P_j = \text{Softmax}(\text{Conv1}\times 1(o_{j}^{dec})),\text{$j\in$[$n$+1,$n$+$p$]}
% P_j = \text{softmax}(\text{Conv1}\times 1([X'_{j};o_{j}^{dec}])),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation}
\end{large}
% \end{normalsize}
% The input to TFN is a squence of the historical turbulence features at multiple previous time stamps $X_1,X_2,..., X_n \in \mathbb{R}^{H\times W\times L \times F}$, where $H\times W\times L$ is the shape of a grid-based 3D region and $F$ is the number of channels/features for each grid. The output of TFN is a squence of the forecasted turbulence conditions $P_1,P_2,\\...,P_n \in \mathbb{R}^{H\times W\times L \times 1}$.
% $X_1^{H\times W\times L \times F},X_2^{H\times W\times L \times F},...,\\ X_n^{H\times W\times L \times F}$
% $X_1,X_2,..., X_n, \belong \mathbb{R}^{H\times W\times L \times F}$
\subsection{Turbulence Detection Network}
The Turbulence Detection Network (TDN) employs \ti{Convolutional Neural Network} to extract sptial correlations and predict the turbulence conditions. The input to TDN is the NWP forecasted turbulence feature cube $X_i$ at time stamp $i$, and the output is the detected turbulence level cube at the same time stamp $P_i \in \mathbb{R}^{\mc{L\times W\times H } \times 4}$. TDN can be summarized as equation (11)-(13):
\begin{large}
\begin{equation}
\text{Conv}(X_{i},1) = f_1(X_i*W_1+b_1)
\end{equation}
\begin{equation}
\text{Conv}(X_{i},l) = f_l(\text{Conv}(X_{i},l-1)*W_l+b_l)
\end{equation}
\begin{equation}
P_i = \text{Softmax}(\text{Conv}(X_{i},l)),\text{$i\in$[$n$+1,$n$+$p$]}
\end{equation}
\end{large}
where $l$ denotes the l-th layer, $f_l$ denotes the activation function of l-th layer, `*' denotes the convolution operator.
% One may be confused about why we need to do turbulence detection since our aiming task is turbulence forecasting. 


\subsection{Dual Label Guessing}
As mentioned before, a major challenge of turbulence forecasting is the \ti{label sparsity} issue. Given a specific time stamp, only a small part of the spatial grids are labeled with the turbulence condition. That is, given $Y_i \in \mathbb{R}^{\mc{L\times W\times H} \times 4}$, most grids in $Y_i$ are unknown. Consequently, we have to mask these unlabeled grids during training to avoid the propagation of their gradients. This leads to less available training signals and the network may not be trained sufficiently. 

In order to mitigate this issue, we propose a novel \ti{Dual Label Guessing} (DLG) method, as shown in Figure \ref{dual}. During the training process, DLG will generate `pseudo-labels' for those unlabeled grids based on TDN and TFN, then these 'pseudo-labels' are coupled with the corresponding features as ground truth and added into the training data. To highlight, DLG differs from other exisiting 'label-guessing' methods \cite{lee2013pseudo, berthelot2019mixmatch} in two fundamental ways:
\begin{itemize}[leftmargin=*]
% \item \ti{\tb{Complementary Dual Information Source.}}
\item \ti{\tb{Complementary Dual Semi-supervised Signals.}}
Instead of \ti{single source} inference, our method leverages \ti{dual source} signals from two related but different tasks.
According to ensemble learning theory \cite{dietterich2002ensemble}, ``\ti{two heads are better than one}"", integrating multiple diversified models as a \ti{committee} could help make more robust predictions. DGL uses a elaborate \ti{Dynamic Ensemble} method to fuse the
% two semi-supervised signals, i.e., 
predictions from TDN and TFN, protecting each other from their individual errors/bias, thus getting more robust to generate high-quality pseudo-labels.   

% With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels.
% However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. 
% Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. 

% To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. \\ 
\item \ti{\tb{Soft Labels.}} Instead of the \ti{hard label} in other approaches like ``pseudo-labeling" \cite{lee2013pseudo} which takes the class with the highest probabilty and produce a one-hot label, we adopt \ti{soft label} via a "sharpening" function \cite{berthelot2019mixmatch}. Compared with the hard label, the soft label is smoother and error-tolerant. Accordingly, a novel \ti{weighted $L2$ loss function} is devised to train it. 

% And which is inspired by the idea of "pseudo-labeling" \cite{lee2013pseudo}. Pseudo-labeling is a semi-supervised learning method which enlarges training set by taking the model's most confident prediction as ground truth added into the set. 

% (1) Instead of single source inference, our method leverages dual source information from two complemenary tasks. With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels. However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. To assist the initial generation, TDN is pretrained in advance. To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. (2) Instead of the hard label in pseudo-labeling which takes the class with the highest probabilty and produce a one-hot label, we adopt soft label via a "sharpening" function \cite{berthelot2019mixmatch}. Compared with the hard label, the soft label is smoother and error-tolerant.

% (3) 
\end{itemize}

\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-7pt}
\centering
\includegraphics[width=0.47\textwidth]{./figures/dual3.pdf}
\vspace{-0.4cm}
\caption{Diagram of Dual Label Guessing.}
\label{dual}
\vspace{-0.1cm}
\end{figure}

\subsubsection{\tb{\large{{Dynamic Ensemble of TDN and TFN}}}}
In our \ti{Dual Label Guessing}, we first propose a novel \ti{Dynamic Ensemble} method to fuse the predictions of TFN and TDN grid by grid, which is defined as: 
% Given $p^{\sss TDN}, p^{\sss TFN} \in \mathbb{R}^{4}$, prediction vectors for a single grid of TDN and TFN respectively,  \ti{Dynamic Ensemble} is defined as:
\begin{large}
\begin{equation}
% p_{ij} = (1-\beta(t))p_{ij}^{\sss TDN}+\beta(t)p_{ij}^{\sss TFN}
% p = (1-\tau(t))p^{\sss TDN}\oplus \tau(t)p^{\sss TFN}
 % p={\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))
 p=\frac{{\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))\oplus {\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))}{2}
\end{equation}
\end{large}
% where $p_{ij}^{\sss TDN}, p_{ij}^{\sss TFN} \in \mathbb{R}^{C}$ are vectors representing the probabilities of each class for the grid $(i,j)$, predicted by TDN and TFN respectively. $C$ is the number of classes, in our case, $C=5$. $\beta(t)$ is a dynamic coefficient controlling the relative importance of TDN and TFN, defined as:
where $p^{\sss TDN}, p^{\sss TFN} \in \mathbb{R}^{4}$ are output vectors for a single grid predicted by TDN and TFN respectively, in which each element represents the probability of each turbulence class. $\oplus$ denotes element-wise addition.
$\xi$ denotes the $\ti{\tb{binary sampling}}$. To be noted, the two ${\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))$ are different samples and $\xi$ is defined as:
\begin{large}
\begin{equation}
\xi(p^{\sss TDN}, p^{\sss TFN},\tau(t)) = \left\{\begin{matrix}
p^{\sss TDN}, & \text{if } r(t) >\tau(t)\\ 
p^{\sss TFN}, & \text{if } r(t)<=\tau(t) 
\end{matrix}\right.
\end{equation}
\end{large}
$r(t)$ above is a \ti{pseudorandom number} between $[0,1]$ with $t$ as the seed. $\tau(t)$ is a \ti{dynamic coefficient} controlling the probability, i.e., \ti{relative importance} of TDN and TFN, $\tau(t)$ is defined as:
\begin{large}
\begin{equation}
\tau(t) = \left\{\begin{matrix}
 0 & t<T_1\\ 
 \frac{t-T_1}{T_2-T_1}\beta & T_1<t<T_2 \\ 
 \beta & T_2>t 
\end{matrix}\right.
\end{equation}
\end{large}

\noindent where $t$ is the number of iterations, $T_1,T_2$ and $\beta$ are the hyperparameters. TDN is chosen to be have higher probability at the beginning of training ($1-\tau(0)=1$ makes TDN 100\% to be chosen), because TDN is \tb{pretrained} and should be more accurate than TFN. As the iteration $t$ increases, TDN's probability is decreasing and TFN's is increasing since TFN's accuracy is growing. Finally the binary sampling probability stabilizes at some balancing point $\beta\in (0,1]$. 

The whole process of DLG is like: when it starts, TDN is dominant in generating the pseudo-labels, and `sharing' its knowledge with TFN through the pseudo-labels; as iterations increase, TFN gradually learns to make good predictions and good `guess', then become balanced with TDN so that and they learn from each other. The balancing ratio is adjusted by $\beta$.


% TDN's weight is decreasing and TFN's is increasing since TFN's accuracy is growing.
\subsubsection{\tb{\large{Soft Labels}}}
After getting the ensembled prediction $p$, to obtain the pseudo-label, we further apply a sharpening function to minimize the \ti{entropy} of the label distribution, which is defined as: 
\begin{large}
\begin{equation}
\text{Sharpen}(p,T)_i := p[i]^{\frac{1}{\sss T}}\Big/\sum_{j=1}^{4}p[j]^{\frac{1}{\sss T}}
\end{equation}
\end{large}
where $p[i]$ is the $i$-th element of $p$, $T$ is a hyperparameter to adjust the ``temperature" of this categorical distribution \cite{goodfellow2016deep}. $\tb{Sharpen}(p,T)$ first calculates the $T$-th power of each elements and then based on which performs a normalization. When $T\rightarrow 0$, the result will approach a one-hot distribution.


\subsection{Label Quality Detector}
Now we have obtained intuitively right pseudo-labels to enlarge training data. 
% \model is partially trained on these pseudo-labels,
The quality of these pseudo-labels is vital to the final performance of our model. More correct labels would produce positive impacts while wrong labels may be destructive to model behavior. In other words, we need to address two questions: (1) how to validate the quality of generated pseudo-labels? (2) how to make better use of "good" pseudo-labels and avoid the "bad" ones?
% But there are two questions still unclear: 1)how good are these generated pseudo-labels? 2) how to make better use of "good" pseudo-labels and avoid the "bad" ones?
To this end, we propose a heuristic \ti{Label Quality Detector} (LQD), to monitor the quality of pseudo-labels and calculate a quality score for each grid. Then, we reassign weight to each grid based on the quality score, grids with high quality scores would have more impact to the loss fuction while grids with low quality contribute less. 

The intuition of LQD is: when TDN and TFN make more \ti{consistent} predictions, the ensembled pseudo-label is more reliable. In other words, the quality is inverse to the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. Specifically, we adopt \ti{Kullback-Leibler Divergence} to measure the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. In order to normalize the score to the range of $[0,1]$, we devise a variant of KL-Divergence, which, given a pseudo-label $p$, is defined as:
% Given a pseudo-label $p$, LQD($p$) 
\begin{large}
\begin{equation}
\text{LQD}(p) = \exp({-D_{KL}(p^{\sss TDN}||p^{\sss TFN})})
\end{equation}
\end{large}
\begin{large}
\begin{equation}
D_{KL}(p^{\sss TDN}||p^{\sss TFN}) = \sum_{i}p_i^{\sss TDN}\log(\frac{p_i^{\sss TDN}}{p_i^{\sss TFN}})
\end{equation}
\end{large}
LQD($p$)=1 when $p^{\sss TDN}$ and $p^{\sss TFN}$ are identical and LQD($p$)$\rightarrow$0 when they are too different. We make use of this quality score by multiplying it with the loss term, see line 11 in Algorithm 1. 
% \subsection{Local Consistency Regularization}
% % forecasting accuracy
% To further improve the label quality, we propose a Local Consistency Regularization method, based on the observation that: turbulence has strong \tb{local continuity} and \tb{correlation}. In other words, adjacent grids tends to have similar turbulence conditions. To implement this intuition, we define the loss function of Local Consistency Regularization as:
% \begin{equation}
% \mc{L}_r = \frac{1}{N_BN_cN_n}\left (\sum_{b=1}^{N_B}\sum_{t=n+1}^{n+p}\sum_{c=1}^{N_c}\sum_{a=1}^{N_a}\left \| p_{btc}^{\sss TFN}-p_{bta}^{\sss TFN} \right \|\right )
% \end{equation}
% where $N_B$ is the number of batches, $p$ is the length of forecasted sequence, $N_c$ is the number of sampled central grids, $N_a$ is the number of adjacent neighbor grids. Specifically, we impose the regularization by the following steps: (1) sample $N_c$ unlabeled grids as "central grids", (2) for each cental gird, ramdomly select $N_a < 27$ grids from its adjacent neighbors,  (3) minimize the L2 distance between the predictions of central grid and neighbor grids. 
\subsection{Loss Functions}
The loss function of our \model includes two parts: (1) $\mc{L}_s$, the supervised part for the labeled grids, (2) $\mc{L}_u$, the unsupervised part for the grids with pseudo-labels. 
\begin{large}
\begin{equation}
\mc{L}=\mc{L}_s+\lambda\mc{L}_u
\end{equation}
\end{large}
where $\lambda\in[0,1]$ is a hyperparameter controlling the weight of unsupervised loss. 

For the supervised loss $\mc{L}_s$, we adopt the Focal Loss \cite{lin2017focal} instead of the Cross Entropy, to handle the label \ti{imbalance} issue.
% because our data is highly \ti{imbalanced} and it is better at handling imbalanced data. 
Given the multiclass prediction $p$ and label $y$, it is defined as:
\begin{large}
\begin{equation}
\text{FC}(p,y)=\sum_{i=1}^4-\text{I}(y_i=1)(1-p_i)^{\gamma}\log(p_i)
\end{equation}
\end{large}
where $(1-p_i)^{\gamma}$ is the ``modulating factor". When an example is misclassified and $p_i$ is small, the modulating factor is near 1 and the loss is unaffected. As $p_i\rightarrow$1, the factor goes to 0 and the loss for well-classified examples (in our case is the majority class of the imbalanced dataset) is down-weighted. The parameter $\gamma$ smoothly adjusts the rate at which easy examples are down-weighted. 
When $\gamma=0$, FL is equivalent to CE. When $\gamma$ is increased, the effect of the modulating factor is likewise increased.

 % penalty term to those ``easy" examples, which, most of the time, is the majority class in a imbalanced dataset.

For the unsupervised loss $\mc{L}_u$, we use the L2 distance since the pseudo-label is a continuous probability distribution instead of one-hot distribution. To alleviate the imbalance issue, we modify L2 to \ti{weighted-L2} by adding a 
weighting factor $\alpha_i\in[0,1]$, which is defined as the normalized \ti{inverse class frequency} (IF):
\begin{large}
\begin{equation}
\alpha_i = \frac{IF_i}{\sum_iIF_i}
\end{equation}
\end{large}
\begin{large}
\begin{equation}
IF_i = \frac{N}{N_i}
\end{equation}
\end{large}
% The final loss is the \ti{weighted-L2 loss}:
\begin{large}
\begin{equation}
\text{weighted-L2}(p,y)=\sqrt{\sum_{i=1}^{4}\alpha_i(p_i-y_i)^2}
\end{equation}
\end{large}
where $N$ is the number of all samples, $N_i$ is the number of samples of class $i$, $IF_i$ is the inverse class frequency. Those majority classes usually have high frequencies and thus get small $\alpha_i$ while minor classes get larger $\alpha_i$, consequently the training speed of the imbalanced data are \ti{rebalanced}.

\subsection{Training \model}
The training process of \model is presented in Algorithm 1. TDN is first pre-trained (Line 6) before the co-training process of TFN and TDN. In every batch, we first obtain the predictions of TDN and TFN via the feedforward network (Line 10-11), then we generate pseudo-labels for unlabeled grids using DLG and obtain the quality score for every pseudo-label using LQD (Line 12-13). Based on these, the the supervised and unsupervised losses are calculated respectively, then we use gradient decent to update the parameters of \model (Line 15-18). This process is repeated until convergence.
\begin{algorithm}[ht]
\caption{Training \model}
\begin{algorithmic}[1]
% $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
\REQUIRE A set of historical turbulence feature sequence $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$.\\
% \ENSURE Trained TFN$(\mc{\theta})$
\ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
\STATE $\text{I}_s=\{\text{mask unlabled grids, keep labeled}\}$.
\STATE $\text{I}_u=\{\text{mask labled grids, keep unlabeled}\}$.
\STATE $\text{T} = \{n+1,...,n+p\}$, the forecasting time stamps.
\STATE Let $\left\|\cdot \right\|_{weighted}$ denote \tb{weighted-L2}.
\STATE Let $\circ$ denote the \tb{Hadamard product}.
\STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
\WHILE{not converge}
% \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
\STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
\FOR {$({X}_h^b,{X}_f^b,{Y}^b) \in \mc{B}$}
\STATE ${P}^{b}_{\sss TFN}=\mc{F}({X}_h^b,{X}_f^b;\theta_{\sss TFN})$;
\STATE ${P}^{b}_{\sss TDN}=\mc{F}({X}_f^b;\theta_{\sss TDN})$;
\STATE Generate pseudo-label $\hat{{Y}}^{b}$ using ${P}^{b}_{\sss TFN},{P}^{b}_{\sss TDN}$ by equation (14)-(17);
\STATE Calculate label quality score $\text{S}^b$ by equation (18)-(19);
\ENDFOR
\STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}({P}^{b,t}_{\sss TFN},{Y}^{b,t}) \right )$
% \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|\right )$
\STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|_{weighted} \right )$
\STATE $\mc{L}=\mc{L}_s+\lambda\mc{L}_u$
\STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
\ENDWHILE
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[ht]
% \caption{Training \model}
% \begin{algorithmic}[1]
% % $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
% \REQUIRE A set of historical turbulence feature sequence $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% % real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
% forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$.\\
% % \ENSURE Trained TFN$(\mc{\theta})$
% \ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
% \STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
% \STATE $\text{I}_s=\{\text{mask unlabled grids}\}$
% \STATE $\text{I}_u=\{\text{mask labled grids}\}$
% \STATE $\text{T} = \{n+1,...,n+p\}$, the forecasting time stamps.
% \WHILE{not converge}
% % \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
% \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% % \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% \FOR {$(\mc{X}_h^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% \STATE $\mc{P}^{b}_{\sss TFN}=\mc{F}(\mc{X}_h^b,\mc{X}_f^b;\theta_{\sss TFN})$;
% \STATE $\mc{P}^{b}_{\sss TDN}=\mc{F}(\mc{X}_f^b;\theta_{\sss TDN})$;
% \STATE Generate pseudo-label $\hat{\mc{Y}}^{b}$ using $\mc{P}^{b}_{\sss TFN},\mc{P}^{b}_{\sss TDN}$ by equation (9)-(11);
% \STATE Calculate label quality score $\mc{S}^b$ by equation (12);
% \ENDFOR
% \STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}(\mc{P}^{b,t}_{\sss TFN},\mc{Y}^{b,t}) \right )$
% \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| \mc{P}^{b,t}_{\sss TFN}-\hat{\mc{Y}}^{b,t} \right \|\right )$
% % \STATE For each $t\in \mc{T}$, sample $N_c$ unlabeled grids as central grids $\mc{C}_t$, for each $c\in \mc{C}_t$, sample $N_a$ adjacent grids as $\mc{A}_c$. 
% % \STATE $\mc{L}_r = \mathlarger{\frac{1}{|\mc{B}||\mc{T}|N_cN_a}} \left (\mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \mc{T}}\mathlarger\sum\limits_{c\in \mc{C}_t}\mathlarger\sum\limits_{a\in \mc{A}_c}\left \| \mc{P}^{b,t,c}_{\sss TFN}-\mc{P}^{b,t,a}_{\sss TFN} \right \|\right )$
% \STATE $\mc{L}=\mc{L}_s+\mc{L}_u$
% \STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
% \ENDWHILE
% \STATE$\circ$ denotes the \tb{Hadamard product}.
% \end{algorithmic}
% \end{algorithm}

==> ICDM20 2/introduction.tex <==
\section{Introduction}
Turbulence is the leading cause of injuries to airline passengers and causes huge loss for airline companies.
%Turbulence forecasting is critical to airline safety and cost control.
According to the U.S. Federal Aviation Administration (FAA), from 1980 through 2008, U.S. air carriers had 234 turbulence accidents, resulting in 298 serious injuries and three fatalities. More lately, since 2009, more than 340 turbulence related injuries have been reported\footnote{https://www.faa.gov/news/fact\_sheets}.
% \footnote{https://www.faa.gov/news/fact\_sheets/news\_story.cfm?newsId=20074}.
% According to the U.S. Federal Aviation Administration (FAA), from 2009 through 2018, U.S. air carriers had 234 turbulence accidents, resulting in 298 serious injuries and three fatalities\footnote{www.faa.gov}. 
The consequent economic losses are enormous. A vice president of one major air carrier once estimated that it pays out ``tens of millions per year'' for customer injuries, and loses about 7000 days in employee injury-related disabilities \cite{sharman2006integrated}. 
If turbulence can be forecasted accurately so that airlines can reroute ahead, then injuries and property damage can be averted, even lives can be saved.


% However, turbulence forecasting is difficult due to being a ``microscale'' phenomenon. 
Despite the benefits, turbulence has been difficult to forecast for being a ``microscale'' phenomenon. 
In the atmosphere, turbulent ``eddies'' vary in size, from hundreds of kilometers down to centimeters. But aircraft bumpiness is most pronounced when the turbulent eddies and aircraft are similar in size. 
It is impossible to directly forecast atmospheric motion at this scale, now or even in the foreseeable future \cite{sharman2006integrated}.
% It is impossible to directly and routinely forecast atmospheric motion at this scale, now or even in the foreseeable future \cite{sharman2006integrated}.  
Fortunately, most of the energy associated with turbulent eddies on this scale cascade down from the larger scales of atmospheric motion \cite{dutton1970clear, tung2003k, koshyk2001horizontal}, and these larger scales may be resolved by Numerical Weather Prediction (NWP) models. 
Based on NWP, a variety of \ti{turbulence indexes}, derived from basic weather features, are proposed by meteorologists to estimate the probability of turbulence occurrence \cite{sharman2006integrated}.
% For reference, \cite{sharman2006integrated} reviewed 13 turbulence indexes and further proposed an integrated approach to combine them for turbulence forecasting.
While most existing turbulence forecasting methods rely on turbulence indexes, however, we observe that solely using manually crafted features is usually suboptimal, yielding unsatisfactory accuracy. 
Moreover, turbulence indexes have poor generalization power to adapt to new data, especially can not handle more complex situations such as climate change.

On the other hand, prior work has shown that a related problem, i.e., weather forecasting can be solved in a more effective and automatic way leveraging deep learning \cite{hsieh2015inferring, xingjian2015convolutional}, 
whereas, researches on applying advanced machine learning models to turbulence forecasting still remain few.
% To this end, we investigate the utility of a variety of machine learning methods on this task, using turbulence events recorded by pilot reports as ground truth labels.
To this end, we make the very first attempt to leverage deep learning for turbulence forecasting, using turbulence events recorded by pilot reports as ground truth labels.
Nevertheless, we find two inevitable challenges impeding us from building an effective turbulence forecasting system:

% \begin{figure*}[htb]
% %\vspace{-0.3cm}
% % \setlength{\textfloatsep}{0.3cm}
% \setlength{\belowcaptionskip}{-7pt}
% \centering
% \includegraphics[width=1\textwidth]{./figures/overview1.png}
% % \includegraphics[width=1\textwidth]{./figures/overview.pdf}
% % \vspace{-0.6cm}
% \caption{Overview of our turbulence forecasting framework}
% % \lyc{duplicate with Figure 2, you can remove it if you are out of space}
% \label{overview}
% % \vspace{-0.1cm}
% \end{figure*}

\begin{itemize}[leftmargin=*]
	\item \noindent\tb{Complex spatio-temporal correlations}. 
	% Turbulence is a disturbance in air movements that typically cannot be seen.
	Turbulence is in nature a \ti{spatio-temporal} phenomenon of air movements. It may occur as a result of various conditions, such as proximity to the jet stream or mountain waves.
% 	thunderstorms. 
	These conditions can actually be captured by certain combinations of meteorological features of the surrounding area and adjacent time slots. Most existing approaches only consider the static features of the target area but neglect the spatio-temporal features of surrounding areas.
	\item \tb{Label scarcity.} Under the paradigm of supervised learning, a large number of turbulence labels are needed to provide signals for training a statistical forecasting model. 
	However, the turbulence label is very \ti{scarce} in the real-world because: (\romannumeral1) turbulence is a rare and anomaly event, (\romannumeral2) it can only be recorded when there is a pilot happens to pass by
% 	it can only be recorded when there is a pilot happens to pass through the same area at the same time of the turbulence. 
	Data with scarce labels, largely limits the power of machine learning.
% 	\item \tb{Label imbalance.} Not only the turbulence labels are hard to collect, but the label distribution is also highly \ti{imbalanced.} According to our statistics of a 7-day's pilot report dataset, only 30\% of the labels are labeled with ``moderate or greater'' (MOG) while only 0.5\% are ``severe''.
% 	Statistical models, trained on the skewed data, usually easily incline to the majority class, causing an unsatisfying performance on the minority classes.

\end{itemize}
% to the jet stream, mountain waves, or convective activity such as thunderstorms or frontal systems. 

To address the above challenges, we present a unified semi-supervised deep learning framework for turbulence forecasting, namely, \model. 
% As shown in Figure \ref{overview}, 
\model~consists of two modules, i.e., a turbulence forecasting model and a turbulence detection model, which are co-trained in a semi-supervised manner.
% Specifically, we first extract historical and forecasted weather features (provided by NWP models) of a spatial region and calculate turbulence indexes to build the feature cubes. 
% (shown in the middle of Figure \ref{overview}). 
% (the latter in Figure \ref{overview})
% Similarly, the label cubes are filled by the extracted sparse turbulence labels.
% Then, an encoder-decoder paradigm, built upon the convolutional LSTM (ConvLSTM), is employed to learn the complex spatio-temporal patterns causing turbulence automatically. 
% Then, an encoder-decoder paradigm, built upon the convolutional LSTM (ConvLSTM), is employed to learn the complex spatio-temporal patterns causing turbulence automatically. 
The forecasting model is built upon ConvLSTM to learn the complex spatio-temporal patterns for causing turbulence automatically.
To take advantage of massive unlabeled data and alleviate the label scarcity issue, 
we propose a novel {Dual Label Guessing} (DLG) method for data augmentation.
In DLG, 
we introduce an auxiliary task, \tb{T}urbulence Detection, and employ 3D-CNN for this task.
% along with the main task of \tb{T}urbulence Forecasting, 
\model~integrates complementary signals from the two tasks to generate more robust pseudo-labels,
% These pseudo-labels are then adopted as ground truth and added into the training loop for better generalization ability. 
which are then utilized as additional data for better generalization ability. 
% Meanwhile, to minimize the effect of ``bad'' pseudo-labels, we propose a heuristic {Label Quality Detector} based on KL-Divergence and re-weighting data by the label quality score. 
% Moreover, to mitigate the label imbalance issue, we devise a {hybrid loss function} consisting of a Focal Loss for the labeled data and weighted-L2 for the pseudo-labels respectively.
% Finally, we create a large-scale real-world turbulence dataset, in which the feature data is collected from NOAA weather records while the label data extracted from public pilot reports. 
% Based on this dataset, 
Finally, we carry out extensive experiments on a real-world dataset to evaluate our model. Results show that \model{} outperforms strong baseline methods in terms of all evaluation metrics (Accuracy, Weighted-Precision, Weighted-Recall, Weighted-F1). Hence the proposed approach can greatly alleviate the problem of spatio-temporal correlation modeling and label scarcity on turbulence forecasting.

% to evaluate the forecasting performance of our \model and various competitive machine learning baselines.
% Experimental 
% Finally, the main contributions of this paper can be summarized as follows:
% \begin{enumerate}
% \item 
% \item 
% \end{enumerate}

==> ICDM20 2/methodology.tex <==
\section{Methodology}
% \lyc{need to highlight the technical contribution, now it looks like a combination of existing methods}
% In this section, we introduce the details of our proposed turbulence forecasting framework, \model. As shown in Figure \ref{framework}, \model{} mainly consists of a \ti{\large{\tb{T}}urbulence Forecasting Network} (\tb{T}FN) and a \ti{\large{\tb{T}}urbulence Detection Network} (\tb{T}DN). 
In this section, we introduce the details of our proposed turbulence forecasting framework, \model. As shown in Figure \ref{framework}, \model{} mainly consists of a \ti{{\tb{T}}urbulence Forecasting Network} (\tb{T}FN) and a \ti{{\tb{T}}urbulence Detection Network} (\tb{T}DN). 
% and a \ti{Dual Label Guessing} module. 
TFN serves for the main task, i.e., forecasting task, while
% forecasting the turbulence conditions at next few hours. 
% TDN serves for the detection task, i.e., an auxiliary task providing clues for accurate pseudo-label generation.
TDN serves for the auxiliary task, i.e., turbulence detection.
% which provides complementary semi-supervised signals for the main task. 
Based on the predictions of TFN and TDN, a novel \ti{\tb{Dual Label Guessing}} approach is proposed to generate more robust pseudo-labels as additional training data. 
% To minimize the effect of ``bad'' pseudo-labels, we re-weighting the grids tagged with pseudo-labels by our heuristic \ti{\tb{Label Quality Detector}} (LQD) based on the quality scores, and add them into training loop dynamically. Finally, we propose a \ti{\tb{hybrid loss function}} consisting of a Focal loss and weighted-L2 loss to alleviate the label imbalance issue.
% \begin{figure}[t]
% %\vspace{-0.3cm}
% % \setlength{\textfloatsep}{0.3cm}
% \setlength{\belowcaptionskip}{-7pt}
% \centering
% \includegraphics[width=0.48\textwidth]{./figures/framework3.pdf}
% \vspace{-0.6cm}
% \caption{Overview of \model.}
% \label{framework}
% \vspace{-0.1cm}
% \end{figure}
\subsection{Turbulence Forecasting Network}
% TFN employs the architecture of ConvLSTM\cite{xingjian2015convolutional} to model the spatio-temporal correlations among the grids. 
TFN is designed on top of the basic ConvLSTM \cite{xingjian2015convolutional} architecture to model the complex spatio-temporal correlations among different spatial grids.
% ConvLSTM is a variation of LSTM to handle spatio-temporal prediction tasks. 
ConvLSTM is a variation of LSTM which extends basic LSTM cell by replacing the fully connected layer with convolution operation in the internal transitions.
% The key equations of ConvLSTM are shown in (3)\text{-}(7) below, where ${X_t, o_t,H_t}$ are the input, output and hidden vectors respectively, ``$\circledast $'' denotes the {3D-convolution} operator and ``$\circ$'' denotes the Hadamard product:
% \begin{large}
% \begin{equation}
% {i_t}=\sigma({W_{xi}\circledast X_t+W_{hi}\circledast H_{t-1}+W_{ci}\circ C_{t-1}+b_i})
% \end{equation}
% \begin{equation}
% {f_t} = \sigma({W_{xf}\circledast X_t+W_{hf}\circledast H_{t-1}+W_{cf}\circ C_{t-1}+b_f})
% \end{equation}
% \begin{equation}
% {C_t} = {f_t}\circ {C_{t-1}} +{i_t}\circ tanh({W_{xc}}\circledast {X_t}+{W_{hc}}\circledast {H_{t-1}}+{b_c})
% \end{equation}
% \begin{equation}
% {o_t} = \sigma({W_{xo}}\circledast {X_t}+{W_{ho}}\circledast {H_{t-1}}+{W_{co}}\circ {C_t+b_o})
% \end{equation}
% \begin{equation}
% {H_t} ={o_t}\circ tanh({C_t})
% \end{equation}
% \end{large}
As shown in Figure \ref{framework}, TFN consists of two ConvLSTMs, serving as the encoder and decoder respectively. 
The encoder takes a sequence of 4D tensors as input, $\bsy{X_1,X_2,...,X_n} \in \mathbb{R}^{\mc{L\times W\times H \times C}}$, i.e., the historical turbulence feature cubes of time slots $1,...,n$. 
% $\mc{L\times W\times H} $ is the shape of a grid-based 3D region and $\mc{C}$ is the number of channels/features for each grid. 
The decoder takes the last hidden state of the encoder as the initial hidden state, and uses \ti{teacher forcing} \cite{goodfellow2016deep} (use previous ground truth $\bsy{Y_{j-1}}$ as the next input to the decoder) to generate a sequence of features corresponding to the forecasting time slots $n+1,...,n+p$. 
The decoder's outputs are then fed into to a $\text{Conv}1\times 1$ block followed with a Softmax layer to produce the forecasted turbulence levels $\bsy{P_{n+1},P_{n+2},...,P_{n+p}} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
% The decoder's outputs are then concatenated with the forecasted turbulence features at multiple forecasting time stamps, $X'_{n+1},X'_{n+2},..., X'_{n+p} \in \mathbb{R}^{\mc{L\times W\times H  \times C}}$, and fed into to a $Conv1\times 1$ block followed with a $softmax$ layer to produce the forecasted turbulence conditions $P_{n+1},P_{n+2},...,P_{n+p} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
% The process of TFN can be summarized in equations (8)-(10):
The process of TFN can be summarized as:
% \begin{normalsize}
%\begin{large}
\begin{equation*}
\bsy{h_i^{enc},o_i^{enc}} = \text{ConvLSTM}^{enc}\big(\bsy{X_{i},h_{i-1}^{enc}}\big), i\in[1,n]
\end{equation*}
\begin{equation*}
\bsy{h_j^{dec},o_j^{dec}} = \text{ConvLSTM}^{dec}\big(\bsy{Y_{j-1}, h_{j-1}^{dec}}\big),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation*}
\begin{equation*}
\bsy{P_j} = \text{Softmax}\big(\text{Conv1}\times 1(\bsy{o_{j}^{dec}})\big),\text{$j\in$[$n$+1,$n$+$p$]}
% P_j = \text{softmax}(\text{Conv1}\times 1([X'_{j};o_{j}^{dec}])),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation*}
%\end{large}
% \end{normalsize}
% The input to TFN is a squence of the historical turbulence features at multiple previous time stamps $X_1,X_2,..., X_n \in \mathbb{R}^{H\times W\times L \times F}$, where $H\times W\times L$ is the shape of a grid-based 3D region and $F$ is the number of channels/features for each grid. The output of TFN is a squence of the forecasted turbulence conditions $P_1,P_2,\\...,P_n \in \mathbb{R}^{H\times W\times L \times 1}$.
% $X_1^{H\times W\times L \times F},X_2^{H\times W\times L \times F},...,\\ X_n^{H\times W\times L \times F}$
% $X_1,X_2,..., X_n, \belong \mathbb{R}^{H\times W\times L \times F}$
\subsection{Turbulence Detection Network}
The Turbulence Detection Network (TDN) employs \ti{Convolutional Neural Network} to extract spatial correlations and detect the turbulence levels. The input to TDN is the NWP forecasted turbulence feature cube $X_i$ at time slot $i$, and the output is the detected turbulence level cube $P_i \in \mathbb{R}^{\mc{L\times W\times H } \times 4}$ at the same time slot. 
% TDN can be summarized in equations (6)-(8):
TDN can be summarized as:
%\begin{large}
\begin{equation}
\text{Conv}\big(\bsy{X_{i}},1\big) = f_1\big(\bsy{X_i}\circledast \bsy{W_1}+b_1\big),
\end{equation}
\begin{equation}
\text{Conv}\big(\bsy{X_{i}},l\big) = f_l\big(\text{Conv}(\bsy{X_{i}},l-1)\circledast \bsy{W_l}+b_l\big),
\end{equation}
\begin{equation}
\bsy{P_i} = \text{Softmax}\big(\text{Conv}(\bsy{X_{i}},l)\big),\text{$i\in$[$n$+1,$n$+$p$]},
\end{equation}
%\end{large}
where $l$ denotes the l-th layer, $f_l$ denotes the activation function of l-th layer, ``$\circledast $'' denotes the {3D-convolution} operator.
% ``*'' denotes the convolution operator.
% One may be confused about why we need to do turbulence detection since our aiming task is turbulence forecasting. 


\subsection{Dual Label Guessing}
% As aforementioned, a major challenge of turbulence forecasting is the \ti{label scarcity} issue. 
% Given a specific timestamp, only a small portion of the spatial grids are labeled with turbulence levels. 
% That is, given $Y_i \in \mathbb{R}^{\mc{L\times W\times H} \times 4}$, most grids in $Y_i$ are unknown. 
% Consequently, we have to mask these unlabeled grids during training to bypass the backpropagation of their gradients. 
% This leads to less training signals available, making it hard for the network to be trained sufficiently. 
To mitigate the label scarcity issue, we propose \ti{Dual Label Guessing} (DLG), as illustrated in Figure \ref{dual}. 
During training, DLG will generate pseudo-labels for those unlabeled grids so that we can obtain additional training data. 
% which are combined with the corresponding features as ground truth and added into the training data dynamically. 
To highlight, DLG differs from existing ``label-guessing'' methods \cite{lee2013pseudo, berthelot2019mixmatch} in two ways:
\begin{itemize}[leftmargin=*]
% \item \ti{\tb{Complementary Dual Information Source.}}
\item \ti{\tb{Complementary Dual Semi-supervised Signals.}}
Instead of \ti{single source} inference, our method leverages \ti{dual source} signals from two related but different tasks.
% According to the ensemble learning theory \cite{dietterich2002ensemble}, ``\ti{two heads are better than one}'', integrating multiple diversified models as a \ti{committee} could help make more robust predictions. 
DLG combines the predictions from TDN and TFN, protecting each other from their individual errors/bias, thus getting more robust to generate high-quality pseudo-labels.   
% two semi-supervised signals, i.e., 
% With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels.
% However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. 
% Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. 

% To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. \\ 
\item \ti{\tb{Soft Labels.}} Instead of the \ti{hard label} in other approaches like ``pseudo-labeling'' \cite{lee2013pseudo} which takes the class with the highest probability and produce a one-hot label, we produce \ti{soft label} via a ``sharpening'' function \cite{berthelot2019mixmatch}, yielding a class distribution. 
The soft label is smoother and more error-tolerant compared with hard label. 
% Accordingly, a novel \ti{weighted $L2$ loss function} is devised to train it. 

% And which is inspired by the idea of "pseudo-labeling" \cite{lee2013pseudo}. Pseudo-labeling is a semi-supervised learning method which enlarges training set by taking the model's most confident prediction as ground truth added into the set. 

% (1) Instead of single source inference, our method leverages dual source information from two complemenary tasks. With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels. However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. To assist the initial generation, TDN is pretrained in advance. To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. (2) Instead of the hard label in pseudo-labeling which takes the class with the highest probabilty and produce a one-hot label, we adopt soft label via a "sharpening" function \cite{berthelot2019mixmatch}. Compared with the hard label, the soft label is smoother and error-tolerant.

% (3) 
\end{itemize}

\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-6pt}
\centering
\includegraphics[width=0.48\textwidth]{./figures/dual1.pdf}
% \vspace{-0.2cm}
\caption{Diagram of dual label guessing}
\label{dual}
\vspace{-0.1cm}
\end{figure}

\subsubsection{\tb{{{Dynamic Ensemble of TDN and TFN}}}}
In our {Dual Label Guessing}, we first propose a novel \ti{Dynamic Ensemble} method to fuse the predictions of TFN and TDN grid by grid, the combined prediction is defined as: 
% Given $p^{\sss TDN}, p^{\sss TFN} \in \mathbb{R}^{4}$, prediction vectors for a single grid of TDN and TFN respectively,  \ti{Dynamic Ensemble} is defined as:
%\begin{large}
\begin{equation}
% p_{ij} = (1-\beta(t))p_{ij}^{\sss TDN}+\beta(t)p_{ij}^{\sss TFN}
% p = (1-\tau(t))p^{\sss TDN}\oplus \tau(t)p^{\sss TFN}
 % p={\bs }(p^{\sss TDN},p^{\sss TFN},\tau(t))
 \bsy{p}=\frac{{\bs }(\bsy{p^{\sss TDN},p^{\sss TFN}},\tau(t))\oplus {\bs }(\bsy{p^{\sss TDN},p^{\sss TFN}},\tau(t))}{2}
\end{equation}
%\end{large}
% where $p_{ij}^{\sss TDN}, p_{ij}^{\sss TFN} \in \mathbb{R}^{C}$ are vectors representing the probabilities of each class for the grid $(i,j)$, predicted by TDN and TFN respectively. $C$ is the number of classes, in our case, $C=5$. $\beta(t)$ is a dynamic coefficient controlling the relative importance of TDN and TFN, defined as:
where $\bsy{p^{\sss TDN}, p^{\sss TFN}} \in \mathbb{R}^{4}$ are output vectors of a single grid predicted by TDN and TFN respectively, in which each element represents the probability of each turbulence class. $\oplus$ denotes element-wise addition.
$\bs$ denotes the $\ti{\tb{binary sampling}}$. 
To be noted, two ${\bs }(\bsy{p^{\sss TDN},p^{\sss TFN}},\tau(t))$ in the equation are different samples and the sampling function $\bs$ is defined as:
%\begin{large}
\begin{equation}
\bs(\bsy{p^{\sss TDN}, p^{\sss TFN}},\tau(t)) = \left\{\begin{matrix}
\bsy{p^{\sss TDN}}, & \text{if } r(t) >\tau(t)\\ 
\bsy{p^{\sss TFN}}, & \text{if } r(t)<=\tau(t) 
\end{matrix}\right.
\end{equation}
%\end{large}
$r(t)$ above is a \ti{pseudorandom number} between $[0,1]$ with $t$ as the seed. 
$\tau(t)$ is a \ti{dynamic coefficient} controlling the probability of drawing $\bsy{p^{\sss TDN}}$ or $\bsy{p^{\sss TFN}}$ , i.e., \ti{relative importance} of TDN and TFN, $\tau(t)$ is defined as a piece-wise function:
%\begin{large}
\begin{equation}
\tau(t) = \left\{\begin{matrix}
 0 & t<T_1\\ 
 \frac{t-T_1}{T_2-T_1}\beta & T_1<t<T_2 \\ 
 \beta & t>T_2 
\end{matrix}\right.
\end{equation}
%\end{large}

\noindent where $t$ is the number of epochs, $T_1,T_2$ and $\beta$ are hyperparameters. 
The design of $\tau(t)$ follows the intuitions:
at the beginning of training, TDN shall have a higher probability  (in the first stage, $1-\tau(0)=1$ makes TDN 100\% to be chosen), because TDN is pre-trained, predicting more accurately than TFN. 
As the iteration $t$ increases gradually, TDN's probability should decrease and TFN's increases since TFN's accuracy is growing. 
Finally, the binary sampling probability stabilizes at some balancing point $\beta\in (0,1]$.

% To summary, the whole process of DLG is like: when it starts, TDN is dominant in generating the pseudo-labels, and ``sharing'' its knowledge with TFN through the pseudo-labels; 
% as iterations increase, TFN gradually learns to make good predictions and good ``guess'', then become balanced with TDN so that they learn from each other, yielding more robust pseudo-labels.
% The balancing ratio is controllable with the hyper-parameter, $\beta$. 

% TDN's weight is decreasing and TFN's is increasing since TFN's accuracy is growing.
\subsubsection{\tb{Soft Labels}}
After getting the ensembled prediction $p$, to obtain the pseudo-label, we further apply a sharpening function to minimize the \ti{entropy} of the label distribution, which is defined as: 
%\begin{large}
\begin{equation}
\text{Sharpen}(\bsy{p},T)_i := \bsy{p}[i]^{\frac{1}{\sss T}}\Big/\sum_{j=1}^{4}\bsy{p}[j]^{\frac{1}{\sss T}}
\end{equation}
%\end{large}
where $\bsy{p}[i]$ is the $i$-th element of $\bsy{p}$, $T$ is a hyper-parameter to adjust the ``temperature'' of this categorical distribution. $\tb{Sharpen}(\bsy{p},T)$ first calculates the $T$-th power of each elements and then based on which performs a normalization. When $T\rightarrow 0$, the result will approach a one-hot distribution.


% \subsection{Label Quality Detector}
% Now we have obtained pseudo-labels of unlabeled grids to supplement training data. 
% However, the quality of these pseudo-labels, which is vital to the final performance of our model, remains unknown. 
% More correct labels would produce positive impacts while wrong labels are destructive to model behavior. 
% In other words, we need to address two questions: (1) how to validate the quality of generated pseudo-labels? (2) how to make better use of ``good'' pseudo-labels and avoid the ``bad'' ones?
% To this end, we propose a heuristic \ti{Label Quality Detector} (LQD), to monitor the quality of pseudo-labels and calculate a quality score for each grid. 
% Next, we reassign weight to each grid based on the quality score, grids with high-quality scores would have more impact on the loss function while grids with low quality impact less. 

% The intuition of LQD is: when TDN and TFN make more \ti{consistent} predictions, the ensembled pseudo-label is more reliable. In other words, the quality is inverse to the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. Specifically, we adopt \ti{Kullback-Leibler Divergence} to measure the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. 
% % However, the
% Moreover, in order to normalize the score to the range of $[0,1]$, we devise a variation of KL-Divergence, which, given the pseudo-labels $p^{\sss TDN}$ and $p^{\sss TFN}$, is defined as:
% % Given a pseudo-label $p$, LQD($p$) 
% %\begin{large}
% \begin{equation}
% \text{LQD}(p) = \exp({-D_{KL}(p^{\sss TDN}||p^{\sss TFN})})
% \end{equation}
% %\end{large}
% %\begin{large}
% \begin{equation}
% D_{KL}(p^{\sss TDN}||p^{\sss TFN}) = \sum_{i}p_i^{\sss TDN}\log(\frac{p_i^{\sss TDN}}{p_i^{\sss TFN}})
% \end{equation}
% %\end{large}
% LQD($p$)=1 when $p^{\sss TDN}$ and $p^{\sss TFN}$ are identical and LQD($p$)$\rightarrow$0 when the difference is significant.
% % when they differ too much.
% % when they are too different. 
% We make use of this quality score by multiplying it with the loss term, see detail in line 11 of Algorithm 1. 
% % \subsection{Local Consistency Regularization}
% % % forecasting accuracy
% % To further improve the label quality, we propose a Local Consistency Regularization method, based on the observation that: turbulence has strong \tb{local continuity} and \tb{correlation}. In other words, adjacent grids tends to have similar turbulence conditions. To implement this intuition, we define the loss function of Local Consistency Regularization as:
% % \begin{equation}
% % \mc{L}_r = \frac{1}{N_BN_cN_n}\left (\sum_{b=1}^{N_B}\sum_{t=n+1}^{n+p}\sum_{c=1}^{N_c}\sum_{a=1}^{N_a}\left \| p_{btc}^{\sss TFN}-p_{bta}^{\sss TFN} \right \|\right )
% % \end{equation}
% % where $N_B$ is the number of batches, $p$ is the length of forecasted sequence, $N_c$ is the number of sampled central grids, $N_a$ is the number of adjacent neighbor grids. Specifically, we impose the regularization by the following steps: (1) sample $N_c$ unlabeled grids as "central grids", (2) for each cental gird, ramdomly select $N_a < 27$ grids from its adjacent neighbors,  (3) minimize the L2 distance between the predictions of central grid and neighbor grids. 
\subsection{Loss Function}
The loss function of our \model{} includes two parts: (1) $\mc{L}_s$, the supervised part for the labeled grids, (2) $\mc{L}_u$, the unsupervised part for the grids with pseudo-labels. 
%\begin{large}
\begin{equation}
\mc{L}=\mc{L}_s+\lambda\mc{L}_u
\end{equation}
%\end{large}
where $\lambda\in[0,1]$ is a hyperparameter controlling the weight of unsupervised loss. For $\mc{L}_s$, we adopt cross-entropy, and for $\mc{L}_u$ , we employ the L2 distance between model predictions and pseudo labels.

% For the supervised loss $\mc{L}_s$, we adopt the Focal Loss (FL) \cite{lin2017focal} instead of the Cross Entropy (CE), to handle the label \ti{imbalance} issue.
% % because our data is highly \ti{imbalanced} and it is better at handling imbalanced data. 
% Given the multiclass prediction $p$ and true label $y$ of a grid, it is defined as:
% %\begin{large}
% \begin{equation}
% \text{FC}(p,y)=\sum_{i=1}^4-\text{I}(y_i=1)(1-p_i)^{\gamma}\log(p_i)
% \end{equation}
% %\end{large}
% where $(1-p_i)^{\gamma}$ is the ``modulating factor''. When an instance is misclassified and $p_i$ is small, the modulating factor is near 1 and the loss is unaffected. 
% As $p_i\rightarrow$1, the factor goes to 0 and the loss for well-classified instances (in our case is the majority class of the imbalanced dataset) is down-weighted. 
% The parameter $\gamma$ smoothly adjusts the rate at which easy samples are down-weighted. 
% When $\gamma=0$, FL is equivalent to CE. 
% When $\gamma$ increases, the effect of the modulating factor also increases.


% \begin{figure*}
% % \abovecaptionskip
% % \belowcaptionskip
% % \setlength{\belowcaptionskip}{-10pt}
% \subfigure[V-component of wind]{\label{a1}\includegraphics[trim=0 20 0 40, clip, width=4.2cm]{./figures/visual-1.pdf}}
% \subfigure[Temporature]{\label{a2}\includegraphics[trim=0 20 0 40, clip, width=4.2cm]{./figures/visual-2.pdf}}
% \subfigure[Vertical velocity]{\label{a2}\includegraphics[trim=0 20 0 40, clip, width=4.2cm]{./figures/visual-3.pdf}}
% \subfigure[Relative humidity]{\label{a2}\includegraphics[trim=0 20 0 40, clip, width=4.2cm]{./figures/visual-4.pdf}}  
% % \vspace{-4mm}
% \caption{Visualization of the weather data.}\label{visualization}
% % \vspace{-6mm}
% \end{figure*}

% For the unsupervised loss $\mc{L}_u$, L2 distance is more suitable than Cross Entropy since the pseudo-label is a continuous probability distribution rather than one-hot distribution. 
% Still, to alleviate the imbalance issue, we modify L2 to \ti{weighted-L2} by adding a 
% weighting factor $\alpha_i\in[0,1]$, which is defined as the normalized \ti{inverse class frequency} (IF):
% %\begin{large}
% \begin{equation}
% \alpha_i = \frac{IF_i}{\sum_{i=1}^{4}IF_i}
% \end{equation}
% %\end{large}
% %\begin{large}
% \begin{equation}
% IF_i = \frac{N}{N_i}
% \end{equation}
% %\end{large}
% % The final loss is the \ti{weighted-L2 loss}:
% %\begin{large}
% \begin{equation}
% \text{weighted-L2}(p,y)=\sqrt{\sum_{i=1}^{4}\alpha_i(p_i-y_i)^2}
% \end{equation}
% %\end{large}
% where $N$ is the number of all samples, $N_i$ is the number of samples of class $i$, $IF_i$ is the inverse class frequency. Those majority classes usually have high frequencies and thus get small $\alpha_i$ while minor classes get larger $\alpha_i$, consequently the training speed of the imbalanced data are \ti{rebalanced}.




% \subsection{Training \model}
% The training process of \model{} is presented in Algorithm 1. 
% TDN is first pre-trained (Line 6) before the co-training process of TFN and TDN. 
% In each batch, we first obtain the predictions of TDN and TFN via the feedforward network (Line 10-11), then we generate pseudo-labels for unlabeled grids using DLG and obtain the quality score for every pseudo-label using LQD (Line 13-14). 
% Based on these, the supervised and unsupervised losses are calculated respectively and we use gradient descent to update the parameters of \model{} (Line 16-19). 
% This process is repeated until convergence. After training, we use the dynamic ensemble $P^b$ as the final prediction.
% \begin{algorithm}
% \caption{Training \model}
% \begin{algorithmic}[1]
% % $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
% \REQUIRE Historical turbulence feature sequence set $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% % real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
% forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$, the shape of feature/label cube ($L,W,H$), the forecasting time stamps $\text{T} = \{n+1,...,n+p\}$.\\
% % \ENSURE Trained TFN$(\mc{\theta})$
% \ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
% \STATE $\text{I}_s=\{\text{mask unlabled grids, keep labeled}\}$.
% \STATE $\text{I}_u=\{\text{mask labled grids, keep unlabeled}\}$.
% % \STATE $L\times W\times H = 10\times 10\times 5$.
% \STATE Let $\left\|\cdot \right\|_{w}$ denote the \tb{weighted-L2}.
% % \STATE Let $\left\|\cdot \right\|_{weighted}$ denote \tb{weighted-L2}.
% \STATE Let $\circ$ denote the \tb{Hadamard product}.
% % \STATE FC($\cdot$) and $\left\|\cdot \right\|_{w}$ return the element-wise losses of the cube.
% \STATE FC($\cdot$) and $\left\|\cdot \right\|_{w}$ first calculate element-wise losses and then return the cube of losses with shape ($L,W,H$).
% \STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
% \WHILE{not converge}
% % \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
% \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% % \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% \FOR {$({X}_h^b,{X}_f^b,{Y}^b) \in \mc{B}$}
% \STATE ${P}^{b}_{\sss TFN}=\mc{F}({X}_h^b,{X}_f^b;\theta_{\sss TFN})$;
% \STATE ${P}^{b}_{\sss TDN}=\mc{F}({X}_f^b;\theta_{\sss TDN})$;
% \STATE Obtain the ensembled prediction ${P}^{b}$ by equation (14)-(16);
% \STATE Generate pseudo-label $\hat{{Y}}^{b}$ using ${P}^{b}_{\sss TFN},{P}^{b}_{\sss TDN}$ by equation (14)-(17);
% \STATE Calculate label quality scores $\text{S}^b$ by equation (18)-(19);
% \ENDFOR
% % \STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\text{Avg}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\,\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}({P}^{b,t}_{\sss TFN},{Y}^{b,t}) \right )$
% % \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\,\mathlarger\sum\limits_{t\in \text{T}}\,\mathlarger\sum\limits_{i,j,k=1}^{L,W,H} \left[\text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|_{w}\right]_{i,j,k} \right )$
% \STATE $\mc{L}_s =  \mathlarger\sum\limits_{b\in \mc{B}}\,\mathlarger\sum\limits_{t\in \text{T}}\,\mathlarger\sum\limits_{i,j,k=1}^{L,W,H} \left[\text{I}_s\circ \text{FC}({P}^{b,t},{Y}^{b,t})\right]_{i,j,k}  $
% \STATE $\mc{L}_u = \mathlarger\sum\limits_{b\in \mc{B}}\,\mathlarger\sum\limits_{t\in \text{T}}\,\mathlarger\sum\limits_{i,j,k=1}^{L,W,H} \left[\text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}-\hat{{Y}}^{b,t} \right \|_{w}\right]_{i,j,k} $
% % \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|\right )$
% % \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\,\mathlarger\sum\limits_{t\in \text{T}}\,\mathlarger\sum\limits_{i,j,k=1}^{L,W,H} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|_{weighted} \right )$
% \STATE $\mc{L}=\mathlarger{\frac{1}{|\mc{B}||\text{T}| L W H}}\left(\mc{L}_s+\lambda\mc{L}_u\right)$
% % \STATE $\mc{L}=\mc{L}_s+\lambda\mc{L}_u$
% \STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}


% % \begin{algorithm}[ht]
% % \caption{Training \model}
% % \begin{algorithmic}[1]
% % % $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
% % \REQUIRE A set of historical turbulence feature sequence $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% % % real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
% % forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$.\\
% % % \ENSURE Trained TFN$(\mc{\theta})$
% % \ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
% % \STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
% % \STATE $\text{I}_s=\{\text{mask unlabled grids}\}$
% % \STATE $\text{I}_u=\{\text{mask labled grids}\}$
% % \STATE $\text{T} = \{n+1,...,n+p\}$, the forecasting time stamps.
% % \WHILE{not converge}
% % % \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
% % \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% % % \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% % \FOR {$(\mc{X}_h^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% % \STATE $\mc{P}^{b}_{\sss TFN}=\mc{F}(\mc{X}_h^b,\mc{X}_f^b;\theta_{\sss TFN})$;
% % \STATE $\mc{P}^{b}_{\sss TDN}=\mc{F}(\mc{X}_f^b;\theta_{\sss TDN})$;
% % \STATE Generate pseudo-label $\hat{\mc{Y}}^{b}$ using $\mc{P}^{b}_{\sss TFN},\mc{P}^{b}_{\sss TDN}$ by equation (9)-(11);
% % \STATE Calculate label quality score $\mc{S}^b$ by equation (12);
% % \ENDFOR
% % \STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}(\mc{P}^{b,t}_{\sss TFN},\mc{Y}^{b,t}) \right )$
% % \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| \mc{P}^{b,t}_{\sss TFN}-\hat{\mc{Y}}^{b,t} \right \|\right )$
% % % \STATE For each $t\in \mc{T}$, sample $N_c$ unlabeled grids as central grids $\mc{C}_t$, for each $c\in \mc{C}_t$, sample $N_a$ adjacent grids as $\mc{A}_c$. 
% % % \STATE $\mc{L}_r = \mathlarger{\frac{1}{|\mc{B}||\mc{T}|N_cN_a}} \left (\mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \mc{T}}\mathlarger\sum\limits_{c\in \mc{C}_t}\mathlarger\sum\limits_{a\in \mc{A}_c}\left \| \mc{P}^{b,t,c}_{\sss TFN}-\mc{P}^{b,t,a}_{\sss TFN} \right \|\right )$
% % \STATE $\mc{L}=\mc{L}_s+\mc{L}_u$
% % \STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
% % \ENDWHILE
% % \STATE$\circ$ denotes the \tb{Hadamard product}.
% % \end{algorithmic}
% % \end{algorithm}


==> ICDM20 2/preliminary.tex <==
\section{Preliminary}
In this section, we introduce several essential preliminaries. First, we give the problem formulation of turbulence forecasting as well as the auxiliary task, turbulence detection. Then we elaborate the features and labels used in our framework. 
% Finally, we elaborate on the challenges found in this task via statistics.
% \begin{figure*}[t]
% %\vspace{-0.3cm}
% % \setlength{\textfloatsep}{0.3cm}
% \setlength{\belowcaptionskip}{-7pt}
% \centering
% \includegraphics[width=1\textwidth]{./figures/overview.png}
% \vspace{-0.4cm}
% \caption{Overview of Our Turbulence Forecasting Framework.}
% \label{overview}
% \vspace{-0.1cm}
% \end{figure*}
\subsection{Turbulence Forecasting}
% We formulate the turbulence forecasting problem as a \ti{sequence to sequence multi-class classification} problem. That is to say, given the historical feature cubes (a cube representing a grid-based 3D region) at previous time slots, $X_1,X_2,...,X_n\in \mathbb{R}^{\mc{L\times W\times H\times C}}$, we aim to predict the turbulence conditions of all grids in this 3D region at next few time slots, i.e.,  $Y_{n+1},Y_{n+2},...,Y_{n+p}\in \mathbb{R}^{\mc{L\times W\times H\times}4}$. $\rm \mc{L\times W\times H}$ is the size (number of grids) of the 3D region, $C$ is the number of channels/features per grid, and $4$ denotes the number of turbulence classes. Each time slot could be, for example, an hour, 3 hours, or a day. In this paper, we choose an hour as the length of a time slot and set $\rm \mc{L\times W\times H}=10\times 10\times 5$, $n=7$, $p=7$, i.e., we use previous 7 hours' feature cubes to forecast the turbulence level of next 7 hours. In Figure \ref{overview}, the bottom right shows an illustration of turbulence forecasting.\lyc{reviewers will ask why 7 hours? and how to choose these hyper parameters?}
We formulate the turbulence forecasting problem as a \ti{sequence to sequence multi-class classification} problem. 
That is, given the historical feature cubes (each cube representing a grid-based 3D region) at previous time slots, $\bsy{X_1,X_2,...,X_n}\in \mathbb{R}^{\mc{L\times W\times H\times C}}$, it aims to predict the turbulence levels of all grids in this 3D region at next few time slots, i.e.,  $\bsy{Y_{n+1},Y_{n+2},...,Y_{n+p}}\in \mathbb{R}^{\mc{L\times W\times H\times}4}$. 
% That is to say, given the historical feature cubes (a cube representing a grid-based 3D region) at previous time slots, $\bsy{X_i,X_2,...,X_n}\in \mathbb{R}^{\mc{L\times W\times H\times C}}$, it aims to predict the turbulence levels of all grids in this 3D region at next few time slots, i.e.,  $Y_{n+1},Y_{n+2},...,Y_{n+p}\in \mathbb{R}^{\mc{L\times W\times H\times}4}$. 
$\rm \mc{L\times W\times H}$ indicates the size (number of grids) of the 3D region, $C$ is the number of channels/features per grid, and $4$ denotes the number of turbulence classes. 
Each time slot could be, for example, an hour, 3 hours, or a day.
Let $\bsy{X}=[\bsy{X_1,X_2,...,X_n}]$, $\bsy{Y}=[\bsy{Y_{n+1},Y_{n+2},...,Y_{n+p}}]$, 
% according to the theory of \ti{Empirical Risk Minimization} (ERM) \cite{vapnik1992principles},  
we aim to train a statistical model $\mc{F}(\cdot;\theta_{TFN})$, that, given $\bsy{X}$, yields a forecast sequence $\bsy{{P}_{\sss TFN}}$ fitting $\bsy{Y}$:
% and perform well on unseen data:
%\begin{large}
\begin{equation}
% \bsy{{P}_{\sss TFN}}=\mc{F}(\bsy{X_h},{X}_f;\theta_{\sss TFN})
\bsy{{P}_{\sss TFN}}=\mc{F}(\bsy{X};\theta_{\sss TFN})
\end{equation}
%\end{large}
% \lyc{also need to mention the forecasted features here}
In this paper, we set $\rm \mc{L\times W\times H}=10\times 10\times 5$ for computation efficiency and flexibility\footnote{The receptive field of $10\times 10\times 5$ is large enough since each grid has the size of 13km, and turbulence ``eddies'' are normally smaller than 100km \cite{sharman2006integrated}.}. We choose one hour as the length of a time slot,
% and set $n=7$, $p=7$, i.e., we use previous 7 hours' feature cubes to forecast the hourly turbulence level of next 7 hours. 
in other words, we use the previous $n$ hours' feature cubes to forecast the hourly turbulence level of next $p$ hours. 
% In Figure \ref{overview}, the bottom right shows an illustration of turbulence forecasting.
% \lyc{7, to be updated}
% \lyc{reviewers will ask why 7 hours? and how to choose these hyper parameters?}

\subsection{Turbulence Detection}
Turbulence detection is a similar task to forecasting which serves as an auxiliary task in \model. 
Given the NWP forecasted feature cube of a time slot $i$, i.e., $\bsy{X_i}\in \mathbb{R}^{\mc{L\times W\times H\times C}}$, 
% \lyc{use a different notation for forecasted features}
turbulence detection aims to predict turbulence conditions of all grids in this 3D region at the {same time slot}, i.e., $\bsy{Y_i} \in \mathbb{R}^{\mc{L\times W\times H\times}4}$. 
% According to ERM theory again,
In this task,
we aim to train a statistical model $\mc{F}(\cdot;\theta_{TDN})$, that, given $\bsy{X_i}$, return detection result $\bsy{{P}_{i,\sss TDN}}$ fitting $\bsy{Y_i}$:
%\begin{large}
\begin{equation}
% {P}_{\sss TFN}=\mc{F}({X}_h,{X}_f;\theta_{\sss TFN})
\bsy{P}_{i,\sss TDN}=\mc{F}(\bsy{X_i};\theta_{\sss TDN})
\end{equation}
%\end{large}
The detection task differs from forecasting task in two ways: (1) \ti{Synchroneity}, i.e., its features are forecasted based on NWP models and synchronized with the turbulence labels. 
It aims to detect future turbulence using future features while forecasting aims to predict future turbulence using past features.
(2) \ti{Static}, it is also easier since it only predicts one step at one time. 
These two tasks share the same target but have different input features and hold different properties. 
We utilize both turbulence forecasting and detection to provide complementary guidance for the pseudo-label generation. 
% details will be discussed in Section 3. 
\begin{table}
\small
\caption{Raw features and turbulence indexes}
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		Notation&Name&Unit\\
		\hline
		\hline
		$v_{_U}$&U component of wind & $\rm ms^{-1}$\\
		\hline
		$v_{_V}$&V component of wind & $\rm ms^{-1}$\\
		\hline
		$T$&Temperature& $\rm K$\\
		\hline
		$H$&Relative humidity & \% \\
		\hline
		$V$&Vertical velocity& $\rm Pas^{-1}$\\
		\hline
		$P$&Pressure & $\rm Pa$\\
		\hline
		\hline
		$Ri$&Richardson Number&- \\
		\hline
		$CP$&Colson Panofsky Index&$\rm kt^2$ \\
		\hline
		$TI1$&Ellrod Indices&$\rm s^{-2}$ \\
		\hline
		$|v|$&Wind Speed &$\rm ms^{-1}$ \\
		\hline
		$|\bigtriangledown_{H}T|$&Horizontal Temperature Gradient& $\rm Km^{-1}$\\
		\hline
		$|v|DEF$&MOS CAT Probability Predictor & $\rm ms^{-2}$\\
		\hline
	\end{tabular}
\label{feature}
\end{table}
% \begin{table}
% \small
% \caption{Labels on turbulence levels}
% 	\centering
% 	\begin{tabular}{|c|c|c|c|c|}
% 		\hline
% 		Code&/NEG&/LGT&/MOD&/SEV\\
% 		\hline
% 		Name&negative&light&moderate&severe\\
% 		\hline
% 		Proportion(\%)&47.79& 21.55&30.12 &0.54\\
% 		\hline
% 	\end{tabular}
% \label{label}
% \end{table}
\subsection{Features}
In each grid of a feature cube (i.e., $\bsy{X_i}$), we fill it with 12 relevant features (thus $C$=12) as shown in Table \ref{feature}.
The first 6 of them are \ti{raw weather features} while the rest 6 are \ti{turbulence indexes} invented by meteorologists.
Raw features such as temperature, wind component, and pressure can be considered as fundamental features and certain combinations of these features in adjacent areas may contribute to the occurrence of turbulence.
\ti{Deep neural network} such as \ti{convolutional neural network} is capable of learning such complex spatial correlations and it is essential to keep the raw features. 
We further apply 6 turbulence indexes as extra features to enhance the model capacity. 
Most of these indexes are proposed by previous meteorologists,  usually adopted independently or integrated by a weighted sum \cite{sharman2006integrated} in existing turbulence forecasting systems. 
We regard them as prior knowledge and concatenate with raw features. 
% to form each feature grid of the feature cubes.
% The feature data is pu
% We collect the feature data from NOAA.
\subsection{Labels and the scarcity issue}
% Table \ref{label} presents the labels of our task, i.e., the turbulence levels, as well as the proportion of each class in our data. 
% The label indicates the severity of the turbulence, corresponding to a real turbulence event recorded by pilot reports.
% and we can observe that the labels are highly \ti{imbalanced}.
We collect turbulence events data from online pilot reports, each is labeled with a severity level. There are four levels in our data, i.e., Negative, Light, Moderate, and Severe.
After gathering the feature data and label data, we align them by time and space.
% The feature and label data are gathered from NOAA and online pilot reports respectively. 
Details are provided in Section 4.
According to our statistics, at each hour, there are only ${0.05\%}$ grids of North American air space are labeled with a turbulence level while $ {99.95\%}$ are unknown.
% Given a specific timestamp, only a small portion of the spatial grids are labeled with turbulence levels. 
Consequently, we have to mask these unlabeled grids during training to bypass the backpropagation of their gradients. 
This leads to less training signals available, making it hard for the network to be trained sufficiently. 
% \lyc{better separate the contents of subsections C,D into 1. features and 2. labels (and issues of labels)}
%Figure \ref{overview} present an overview of our turbulence forecasting framework. We first extract raw weather features of a spatial region and calculate turbulences indexes to form the feature cubes. Then during training, a turbulence forecasting model and turbulence detection model are co-trained in a semi-supervised manner. Then during forecasting stage, we adopt the forecasting model's output as the final result.



% \begin{table}
% \small
% \caption{Raw features and turbulence indexes adopted.}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Notation&Name&Unit\\
% 		\hline
% 		\hline
% 		$\rm v_{_U}$&U component of wind & $\rm ms^{-1}$\\
% 		\hline
% 		$\rm v_{_V}$&V component of wind & $\rm ms^{-1}$\\
% 		\hline
% 		$\rm T$&Temperature& $\rm K$\\
% 		\hline
% 		$\rm H$&Relative humidity & \% \\
% 		\hline
% 		$\rm V$&Vertical velocity& $\rm Pas^{-1}$\\
% 		\hline
% 		$\rm P$&Pressure & $\rm Pa$\\
% 		\hline
% 		\hline
% 		$\rm Ri$&Richardson Number&- \\
% 		\hline
% 		$\rm CP$&Colson Panofsky Index&$\rm kt^2$ \\
% 		\hline
% 		$\rm TI1$&Ellrod Indices&$\rm s^{-2}$ \\
% 		\hline
% 		$\rm |v|$&Wind Speed &$\rm ms^{-1}$ \\
% 		\hline
% 		$\rm |\bigtriangledown_{H}T|$&Horizontal Temperature Gradient& $\rm Km^{-1}$\\
% 		\hline
% 		$\rm |v|DEF$&MOS CAT Probability Predictor & $\rm ms^{-2}$\\
% 		\hline
% 	\end{tabular}
% \label{feature}
% \end{table}
% In addition, about 50\% of the labeled grids are ``negative'' and only less than 1\% are ``severe''. 
% Hence the label of the turbulence data is extreme \ti{scarce} and highly \ti{imbalanced}. 
% This imposes great challenges to effective turbulence forecasting. 
% First, label scarcity will limit the supervision signals a model can learn from. 
% Second, label imbalance will lead to \ti{class skew}, i.e., a model tends to predict the majority classes. 
% In the next section, we introduce our proposed \model, a semi-supervised model for turbulence forecasting and its technical contributions that alleviate these issues. 
\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-7pt}
\centering
% \includegraphics[width=0.48\textwidth]{./figures/framework5.pdf}
\includegraphics[width=0.48\textwidth]{./figures/framework6.pdf}
% \vspace{-0.6cm}
\caption{The architecture of \model}
\label{framework}
\vspace{-0.1cm}
\end{figure}


==> ICDM20 2/relatedwork.tex <==
\section{Related Work}
% In this section, we first introduce relevant studies on turbulence forecasting, followed by machine learning techniques related to spatio-temporal modeling and semi-supervised learning. 
% and learning on imbalanced data.
% \subsection{Turbulence Forecasting}
Traditional turbulence forecasting approaches mainly focus on devising various turbulence indexes \cite{colson1965index,dutton1980probability,ellrod1992objective}.
% The {Colson-Panofsky} index uses dimensional arguments in a stable atmosphere to estimate clear-air turbulence intensities \cite{colson1965index}.
% The {Richardson number}, a well-known theoretical turbulence indicator, is composed of elements relating to both wind shear and atmospheric stability \cite{stull2012introduction}.
% The {Ellrod TI1} index combines the vertical wind shear and deformation while the Ellrod TI2 index further combines the convergence \cite{ellrod1992objective}. Both Ellrod indexes were designed to forecast turbulence associated with strong wind shear, particularly in areas close to the jetstream.
% Dutton \cite{dutton1980probability} proposed an empirical index which comprises components for horizontal wind shear and vertical wind shear. 
% and the values are stated as the probability of encountering CAT in 100 km of level flight.
% It has been used for many years as forecaster guidance at WAFC London. 
% Based on multiple turbulence indexes, 
Sharman et al. reviewed 13 turbulence indexes and proposed an integrated method combining these features to achieve further improvements \cite{sharman2006integrated}.
% \cite{anwar2020machine} proposed to use the Richardson number as extra features and adopt SVM to adjust the weights.
% For its simplicity, turbulence indexes have been widely used in real-world forecasting systems. 
% Turbulence indexes used individually or collectively have achieved certain effects in real-world forecasting systems. 
%However, most of these work adopt basic statistical methods to combine static features with advanced machine learning methods rarely utilized.
However, as validated in our experiments, methods solely rely on turbulence indexes can not achieve satisfactory performance. 
Our method takes advantage of both turbulence indexes and the power of deep learning to achieve superior performance.
% the methods in this category heavily rely on painstakingly customized statistical methods to calculate the indexes from various static weather features, which are less effective in dynamic and complex weather conditions.
% \subsection{Related Machine Learning Techniques}
% In recent years, we have witnessed a growing interest in applying machine learning to a variety of applications such as urban computing \cite{zhang2019flow,geng2019spatiotemporal,zhang2017deep,yao2018deep} and climate-changing \cite{jia2019spatial,faghmous2015computing,karpatne2016monitoring,nayakspatio,wang2019deep}.
Recent years have witnessed a growing interest in applying machine learning to a variety of spatio-temporal problems \cite{karpatne2016monitoring,yuan2020spatio,xingjian2015convolutional}.
Most of them adopt ConvLSTM to model the spatio-temporal correlations without facing the label scarcity issue.
Particularly, we propose a novel semi-supervised approach to tackle the scarcity issue considering by taking complementary turbulence signals into account.
% For instance, \cite{xingjian2015convolutional} proposed the Convolutional LSTM (ConvLSTM) for precipitation nowcasting. 
% ConvLSTM extends basic LSTM cell by replacing the fully connected layer with convolution operation in the internal transitions, hence obtains the ability of modeling spatial and temporal correlations simultaneously. 
% In terms of semi-supervised learning (SSL), Pseudo-labeling \cite{lee2013pseudo} is an effective heuristic SSL method that takes the model's prediction as ground truth and added into training loop dynamically.
% Lately,  \cite{berthelot2019mixmatch} proposed Mixmatch, a holistic approach which unifies several dominant SSL methods and achieves state-of-the-art results on 4 benchmark datasets.
% Recently, \citeauthor{berthelot2019mixmatch} proposed Mixmatch \cite{berthelot2019mixmatch}, a holistic approach which unifies several dominant SSL methods and achieves state-of-the-art results on 4 benchmark datasets.
% Air Quality Inference model (AQI) is a graph-based semi-supervised learning method for inferring air quality of arbitrary location using very sparse monitoring data \cite{hsieh2015inferring}. 
% Similar to our task, it also faces the challenges of spatio-temporal modeling with label scarcity, but turbulence forecasting is more challenging due to the label imbalance issue, and \model{} further takes it into account. 
% Our work also has a connection with GAN \cite{goodfellow2014generative}, in that we both have two sub-models learning from each other. However, \model{} uses complementary sub-models while GAN uses adversarial ones. 
More recently, some work tries to incorporate physical principles with deep learning to facilitate turbulent flow modeling, however, they are not directly tackling turbulence forecasting, but simulating and predicting certain turbulence variables, e.g., Wang et al. predicts the velocity fields \cite{wang2019towards}.
To our best knowledge, our work is the first systematic machine learning study, that directly forecasts the occurrence of flight turbulence, using sparse turbulence labels extracted from pilot reports as supervision.
% To our best knowledge, our work is the first to systematically utilize advanced machine learning to directly forecast the occurrence of flight turbulence.
% To our best knowledge, our work is the first machine learning study to directly forecast the occurrence of flight turbulence using scarce turbulence labels extracted from pilot reports as ground truth.
 % with a sophisticated machine learning approach.




==> figures/methodology.tex <==
\section{Methodology}
% \lyc{need to highlight the technical contribution, now it looks like a combination of existing methods}
In this section, we introduce the details of our turbulence forecasting framework, \model. As shown in Figure \ref{framework}, \model mainly consists of a \ti{\large{\tb{T}}urbulence Forecasting Network} (\tb{T}FN), a \ti{\large{\tb{T}}urbulence Detection Network} (\tb{T}DN). 
% and a \ti{Dual Label Guessing} module. 
TFN serves for the main task, i.e., forecasting task, while
% forecasting the turbulence conditions at next few hours. 
% TDN serves for the detection task, i.e., an auxiliary task providing clues for accurate pseudo-label generation.
TDN serves for the auxiliary task, i.e., detection task, which provides complementary semi-supervised signals for the main task. Based on the predictions of TFN and TDN, a novel \ti{\tb{Dual Label Guessing}} approach is proposed to fuse these two sources of information to generate more robust pseudo-labels as additional training data. In order to minimize the effect of "bad" pseudo-labels, the grids tagged with pseudo-labels are reweighted by our heuristic \ti{\tb{Label Quality Detector}} (LQD) based on the quality scores, and added into training loop dynamically. 
% To further improve the label quality, a novel Local Consistency Regularization is imposed at the output of TFN.
\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-7pt}
\centering
\includegraphics[width=0.48\textwidth]{./figures/framework2.pdf}
\vspace{-0.6cm}
\caption{Overview of \model.}
\label{framework}
\vspace{-0.1cm}
\end{figure}
\subsection{Turbulence Forecasting Network}
% TFN employs the architecture of ConvLSTM\cite{xingjian2015convolutional} to model the spatiotemporal correlations among the grids. 
TFN is designed on top of the basic ConvLSTM \cite{xingjian2015convolutional} architecture to model the complex spatiotemporal correlations among different spatial grids. ConvLSTM is a variation of LSTM to handle spatiotemporal prediction tasks. It extends basic LSTM cell by replacing the fully connected layer with convolution operatoration in the internal transitions.
The key equations of ConvLSTM are shown in (3)\text{-}(7) below, where $X_t, o_t,H_t$ are the input, output and hidden vectors respectively, `$\circledast $' denotes the \ti{3D-convolution} operator and `$\circ$' denotes the Hadamard product:
% \begin{large}
\begin{equation}
i_t=\sigma(W_{xi}\circledast X_t+W_{hi}\circledast H_{t-1}+W_{ci}\circ C_{t-1}+b_i)
\end{equation}
\begin{equation}
f_t = \sigma(W_{xf}\circledast X_t+W_{hf}\circledast H_{t-1}+W_{cf}\circ C_{t-1}+b_f)
\end{equation}
\begin{equation}
C_t = f_t\circ C_{t-1} +i_t\circ tanh(W_{xc}\circledast X_t+W_{hc}\circledast H_{t-1}+b_c)
\end{equation}
\begin{equation}
o_t = \sigma(W_{xo}\circledast X_t+W_{ho}\circledast H_{t-1}+W_{co}\circ C_t+b_o)
\end{equation}
\begin{equation}
H_t =o_t\circ tanh(C_t)
\end{equation}
% \end{large}
% \begin{equation}
% \begin{aligned}
%     &i_t=\sigma(W_{xi}*X_t+W_{hi}*H_{t-1}+W_{ci}\circ C_{t-1}+b_i)\\
%    & f_t = \sigma(W_{xf}*X_t+W_{hf}*H_{t-1}+W_{cf}\circ C_{t-1}+b_f)\\
%     &C_t = f_t\circ C_{t-1} +i_t\circ tanh(W_{xc}*X_t+W_{hc}*H_{t-1}+b_c)\\
%     &o_t = \sigma(W_{xo}*X_t+W_{ho}*H_{t-1}+W_{co}\circ C_t+b_o)\\
%    & H_t =o_t\circ tanh(C_t)
% \end{aligned}
% \end{equation}
As shown in the bottom part of Figure \ref{framework}, TFN consists of two ConvLSTMs, serving as the encoder and decoder respectively. The encoder takes a squence of 4D tensors as input, i.e., $X_1,X_2,...,X_n \in \mathbb{R}^{\mc{L\times W\times H \times C}}$, the historical turbulence feature cubes of time slot $1,...,n$. $\mc{L\times W\times H} $ is the shape of a grid-based 3D region and $\mc{C}$ is the number of channels/features for each grid. The decoder takes the last hidden state of the encoder as the initial hidden state, and uses \ti{teacher forcing} \cite{goodfellow2016deep} (use previous ground truth $Y_{j-1}$ as the next input to the decoder) to generate a sequence of features corresponding to the forecasting time stamps $n+1,...,n+p$. The decoder's outputs are then fed into to a $\text{Conv}1\times 1$ block followed with a Softmax layer to produce the forecasted turbulence conditions $P_{n+1},P_{n+2},...,P_{n+p} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
% The decoder's outputs are then concatenated with the forecasted turbulence features at multiple forecasting time stamps, $X'_{n+1},X'_{n+2},..., X'_{n+p} \in \mathbb{R}^{\mc{L\times W\times H  \times C}}$, and fed into to a $Conv1\times 1$ block followed with a $softmax$ layer to produce the forecasted turbulence conditions $P_{n+1},P_{n+2},...,P_{n+p} \in \mathbb{R}^{\mc{L\times W\times H\times} 4}$. 
The process of TFN can be summarized in equation (8)-(10):
% \begin{normalsize}
\begin{large}
\begin{equation}
h_i^{enc},o_i^{enc} = \text{ConvLSTM}^{enc}(X_{i},h_{i-1}^{enc}), i\in[1,n]
\end{equation}
\begin{equation}
h_j^{dec},o_j^{dec} = \text{ConvLSTM}^{dec}(Y_{j-1}, h_{j-1}^{dec}),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation}
\begin{equation}
P_j = \text{Softmax}(\text{Conv1}\times 1(o_{j}^{dec})),\text{$j\in$[$n$+1,$n$+$p$]}
% P_j = \text{softmax}(\text{Conv1}\times 1([X'_{j};o_{j}^{dec}])),\text{$j\in$[$n$+1,$n$+$p$]}
\end{equation}
\end{large}
% \end{normalsize}
% The input to TFN is a squence of the historical turbulence features at multiple previous time stamps $X_1,X_2,..., X_n \in \mathbb{R}^{H\times W\times L \times F}$, where $H\times W\times L$ is the shape of a grid-based 3D region and $F$ is the number of channels/features for each grid. The output of TFN is a squence of the forecasted turbulence conditions $P_1,P_2,\\...,P_n \in \mathbb{R}^{H\times W\times L \times 1}$.
% $X_1^{H\times W\times L \times F},X_2^{H\times W\times L \times F},...,\\ X_n^{H\times W\times L \times F}$
% $X_1,X_2,..., X_n, \belong \mathbb{R}^{H\times W\times L \times F}$
\subsection{Turbulence Detection Network}
The Turbulence Detection Network (TDN) employs \ti{Convolutional Neural Network} to extract sptial correlations and predict the turbulence conditions. The input to TDN is the NWP forecasted turbulence feature cube $X_i$ at time stamp $i$, and the output is the detected turbulence level cube at the same time stamp $P_i \in \mathbb{R}^{\mc{L\times W\times H } \times 4}$. TDN can be summarized as equation (11)-(13):
\begin{large}
\begin{equation}
\text{Conv}(X_{i},1) = f_1(X_i*W_1+b_1)
\end{equation}
\begin{equation}
\text{Conv}(X_{i},l) = f_l(\text{Conv}(X_{i},l-1)*W_l+b_l)
\end{equation}
\begin{equation}
P_i = \text{Softmax}(\text{Conv}(X_{i},l)),\text{$i\in$[$n$+1,$n$+$p$]}
\end{equation}
\end{large}
where $l$ denotes the l-th layer, $f_l$ denotes the activation function of l-th layer, `*' denotes the convolution operator.
% One may be confused about why we need to do turbulence detection since our aiming task is turbulence forecasting. 


\subsection{Dual Label Guessing}
As mentioned before, a major challenge of turbulence forecasting is the \ti{label sparsity} issue. Given a specific time stamp, only a small part of the spatial grids are labeled with the turbulence condition. That is, given $Y_i \in \mathbb{R}^{\mc{L\times W\times H} \times 4}$, most grids in $Y_i$ are unknown. Consequently, we have to mask these unlabeled grids during training to avoid the propagation of their gradients. This leads to less available training signals and the network may not be trained sufficiently. 

In order to mitigate this issue, we propose a novel \ti{Dual Label Guessing} (DLG) method, as shown in Figure \ref{dual}. During the training process, DLG will generate `pseudo-labels' for those unlabeled grids based on TDN and TFN, then these 'pseudo-labels' are coupled with the corresponding features as ground truth and added into the training data. To highlight, DLG differs from other exisiting 'label-guessing' methods \cite{lee2013pseudo, berthelot2019mixmatch} in two fundamental ways:
\begin{itemize}[leftmargin=*]
% \item \ti{\tb{Complementary Dual Information Source.}}
\item \ti{\tb{Complementary Dual Semi-supervised Signals.}}
Instead of \ti{single source} inference, our method leverages \ti{dual source} signals from two related but different tasks.
According to ensemble learning theory \cite{dietterich2002ensemble}, ``\ti{two heads are better than one}"", integrating multiple diversified models as a \ti{committee} could help make more robust predictions. DGL uses a elaborate \ti{Dynamic Ensemble} method to fuse the
% two semi-supervised signals, i.e., 
predictions from TDN and TFN, protecting each other from their individual errors/bias, thus getting more robust to generate high-quality pseudo-labels.   

% With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels.
% However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. 
% Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. 

% To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. \\ 
\item \ti{\tb{Soft Labels.}} Instead of the \ti{hard label} in other approaches like ``pseudo-labeling" \cite{lee2013pseudo} which takes the class with the highest probabilty and produce a one-hot label, we adopt \ti{soft label} via a "sharpening" function \cite{berthelot2019mixmatch}. Compared with the hard label, the soft label is smoother and error-tolerant. Accordingly, a novel \ti{weighted $L2$ loss function} is devised to train it. 

% And which is inspired by the idea of "pseudo-labeling" \cite{lee2013pseudo}. Pseudo-labeling is a semi-supervised learning method which enlarges training set by taking the model's most confident prediction as ground truth added into the set. 

% (1) Instead of single source inference, our method leverages dual source information from two complemenary tasks. With such scarce labels available, TFN alone is not able to be well trained so as to generate high-quality pseudo-labels. However, the detection task which uses current meteorological features to detect current turbulence conditions, is an easier task compared with forecasting and should produce more accurate pseudo-labels. Thus we introduce detection as the auxiliary task, and ensemble the detection results with forecasting results to generate more robust pseudo-labels. To assist the initial generation, TDN is pretrained in advance. To be clear, the detection task is only used in our training stage since the current meteorological features are not accessible when forecasting. (2) Instead of the hard label in pseudo-labeling which takes the class with the highest probabilty and produce a one-hot label, we adopt soft label via a "sharpening" function \cite{berthelot2019mixmatch}. Compared with the hard label, the soft label is smoother and error-tolerant.

% (3) 
\end{itemize}

\begin{figure}[t]
%\vspace{-0.3cm}
% \setlength{\textfloatsep}{0.3cm}
\setlength{\belowcaptionskip}{-7pt}
\centering
\includegraphics[width=0.47\textwidth]{./figures/dual3.pdf}
\vspace{-0.4cm}
\caption{Diagram of Dual Label Guessing.}
\label{dual}
\vspace{-0.1cm}
\end{figure}

\subsubsection{\tb{\large{{Dynamic Ensemble of TDN and TFN}}}}
In our \ti{Dual Label Guessing}, we first propose a novel \ti{Dynamic Ensemble} method to fuse the predictions of TFN and TDN grid by grid, which is defined as: 
% Given $p^{\sss TDN}, p^{\sss TFN} \in \mathbb{R}^{4}$, prediction vectors for a single grid of TDN and TFN respectively,  \ti{Dynamic Ensemble} is defined as:
\begin{large}
\begin{equation}
% p_{ij} = (1-\beta(t))p_{ij}^{\sss TDN}+\beta(t)p_{ij}^{\sss TFN}
% p = (1-\tau(t))p^{\sss TDN}\oplus \tau(t)p^{\sss TFN}
 % p={\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))
 p=\frac{{\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))\oplus {\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))}{2}
\end{equation}
\end{large}
% where $p_{ij}^{\sss TDN}, p_{ij}^{\sss TFN} \in \mathbb{R}^{C}$ are vectors representing the probabilities of each class for the grid $(i,j)$, predicted by TDN and TFN respectively. $C$ is the number of classes, in our case, $C=5$. $\beta(t)$ is a dynamic coefficient controlling the relative importance of TDN and TFN, defined as:
where $p^{\sss TDN}, p^{\sss TFN} \in \mathbb{R}^{4}$ are output vectors for a single grid predicted by TDN and TFN respectively, in which each element represents the probability of each turbulence class. $\oplus$ denotes element-wise addition.
$\xi$ denotes the $\ti{\tb{binary sampling}}$. To be noted, the two ${\xi }(p^{\sss TDN},p^{\sss TFN},\tau(t))$ are different samples and $\xi$ is defined as:
\begin{large}
\begin{equation}
\xi(p^{\sss TDN}, p^{\sss TFN},\tau(t)) = \left\{\begin{matrix}
p^{\sss TDN}, & \text{if } r(t) >\tau(t)\\ 
p^{\sss TFN}, & \text{if } r(t)<=\tau(t) 
\end{matrix}\right.
\end{equation}
\end{large}
$r(t)$ above is a \ti{pseudorandom number} between $[0,1]$ with $t$ as the seed. $\tau(t)$ is a \ti{dynamic coefficient} controlling the probability, i.e., \ti{relative importance} of TDN and TFN, $\tau(t)$ is defined as:
\begin{large}
\begin{equation}
\tau(t) = \left\{\begin{matrix}
 0 & t<T_1\\ 
 \frac{t-T_1}{T_2-T_1}\beta & T_1<t<T_2 \\ 
 \beta & T_2>t 
\end{matrix}\right.
\end{equation}
\end{large}

\noindent where $t$ is the number of iterations, $T_1,T_2$ and $\beta$ are the hyperparameters. TDN is chosen to be have higher probability at the beginning of training ($1-\tau(0)=1$ makes TDN 100\% to be chosen), because TDN is \tb{pretrained} and should be more accurate than TFN. As the iteration $t$ increases, TDN's probability is decreasing and TFN's is increasing since TFN's accuracy is growing. Finally the binary sampling probability stabilizes at some balancing point $\beta\in (0,1]$. 

The whole process of DLG is like: when it starts, TDN is dominant in generating the pseudo-labels, and `sharing' its knowledge with TFN through the pseudo-labels; as iterations increase, TFN gradually learns to make good predictions and good `guess', then become balanced with TDN so that and they learn from each other. The balancing ratio is adjusted by $\beta$.


% TDN's weight is decreasing and TFN's is increasing since TFN's accuracy is growing.
\subsubsection{\tb{\large{Soft Labels}}}
After getting the ensembled prediction $p$, to obtain the pseudo-label, we further apply a sharpening function to minimize the \ti{entropy} of the label distribution, which is defined as: 
\begin{large}
\begin{equation}
\text{Sharpen}(p,T)_i := p[i]^{\frac{1}{\sss T}}\Big/\sum_{j=1}^{4}p[j]^{\frac{1}{\sss T}}
\end{equation}
\end{large}
where $p[i]$ is the $i$-th element of $p$, $T$ is a hyperparameter to adjust the ``temperature" of this categorical distribution \cite{goodfellow2016deep}. $\tb{Sharpen}(p,T)$ first calculates the $T$-th power of each elements and then based on which performs a normalization. When $T\rightarrow 0$, the result will approach a one-hot distribution.


\subsection{Label Quality Detector}
Now we have obtained intuitively right pseudo-labels to enlarge training data. 
% \model is partially trained on these pseudo-labels,
The quality of these pseudo-labels is vital to the final performance of our model. More correct labels would produce positive impacts while wrong labels may be destructive to model behavior. In other words, we need to address two questions: (1) how to validate the quality of generated pseudo-labels? (2) how to make better use of "good" pseudo-labels and avoid the "bad" ones?
% But there are two questions still unclear: 1)how good are these generated pseudo-labels? 2) how to make better use of "good" pseudo-labels and avoid the "bad" ones?
To this end, we propose a heuristic \ti{Label Quality Detector} (LQD), to monitor the quality of pseudo-labels and calculate a quality score for each grid. Then, we reassign weight to each grid based on the quality score, grids with high quality scores would have more impact to the loss fuction while grids with low quality contribute less. 

The intuition of LQD is: when TDN and TFN make more \ti{consistent} predictions, the ensembled pseudo-label is more reliable. In other words, the quality is inverse to the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. Specifically, we adopt \ti{Kullback-Leibler Divergence} to measure the difference between $p^{\sss TDN}$ and $p^{\sss TFN}$. In order to normalize the score to the range of $[0,1]$, we devise a variant of KL-Divergence, which, given a pseudo-label $p$, is defined as:
% Given a pseudo-label $p$, LQD($p$) 
\begin{large}
\begin{equation}
\text{LQD}(p) = \exp({-D_{KL}(p^{\sss TDN}||p^{\sss TFN})})
\end{equation}
\end{large}
\begin{large}
\begin{equation}
D_{KL}(p^{\sss TDN}||p^{\sss TFN}) = \sum_{i}p_i^{\sss TDN}\log(\frac{p_i^{\sss TDN}}{p_i^{\sss TFN}})
\end{equation}
\end{large}
LQD($p$)=1 when $p^{\sss TDN}$ and $p^{\sss TFN}$ are identical and LQD($p$)$\rightarrow$0 when they are too different. We make use of this quality score by multiplying it with the loss term, see line 11 in Algorithm 1. 
% \subsection{Local Consistency Regularization}
% % forecasting accuracy
% To further improve the label quality, we propose a Local Consistency Regularization method, based on the observation that: turbulence has strong \tb{local continuity} and \tb{correlation}. In other words, adjacent grids tends to have similar turbulence conditions. To implement this intuition, we define the loss function of Local Consistency Regularization as:
% \begin{equation}
% \mc{L}_r = \frac{1}{N_BN_cN_n}\left (\sum_{b=1}^{N_B}\sum_{t=n+1}^{n+p}\sum_{c=1}^{N_c}\sum_{a=1}^{N_a}\left \| p_{btc}^{\sss TFN}-p_{bta}^{\sss TFN} \right \|\right )
% \end{equation}
% where $N_B$ is the number of batches, $p$ is the length of forecasted sequence, $N_c$ is the number of sampled central grids, $N_a$ is the number of adjacent neighbor grids. Specifically, we impose the regularization by the following steps: (1) sample $N_c$ unlabeled grids as "central grids", (2) for each cental gird, ramdomly select $N_a < 27$ grids from its adjacent neighbors,  (3) minimize the L2 distance between the predictions of central grid and neighbor grids. 
\subsection{Loss Functions}
The loss function of our \model includes two parts: (1) $\mc{L}_s$, the supervised part for the labeled grids, (2) $\mc{L}_u$, the unsupervised part for the grids with pseudo-labels. 
\begin{large}
\begin{equation}
\mc{L}=\mc{L}_s+\lambda\mc{L}_u
\end{equation}
\end{large}
where $\lambda\in[0,1]$ is a hyperparameter controlling the weight of unsupervised loss. 

For the supervised loss $\mc{L}_s$, we adopt the Focal Loss \cite{lin2017focal} instead of the Cross Entropy, to handle the label \ti{imbalance} issue.
% because our data is highly \ti{imbalanced} and it is better at handling imbalanced data. 
Given the multiclass prediction $p$ and label $y$, it is defined as:
\begin{large}
\begin{equation}
\text{FC}(p,y)=\sum_{i=1}^4-\text{I}(y_i=1)(1-p_i)^{\gamma}\log(p_i)
\end{equation}
\end{large}
where $(1-p_i)^{\gamma}$ is the ``modulating factor". When an example is misclassified and $p_i$ is small, the modulating factor is near 1 and the loss is unaffected. As $p_i\rightarrow$1, the factor goes to 0 and the loss for well-classified examples (in our case is the majority class of the imbalanced dataset) is down-weighted. The parameter $\gamma$ smoothly adjusts the rate at which easy examples are down-weighted. 
When $\gamma=0$, FL is equivalent to CE. When $\gamma$ is increased, the effect of the modulating factor is likewise increased.

 % penalty term to those ``easy" examples, which, most of the time, is the majority class in a imbalanced dataset.

For the unsupervised loss $\mc{L}_u$, we use the L2 distance since the pseudo-label is a continuous probability distribution instead of one-hot distribution. To alleviate the imbalance issue, we modify L2 to \ti{weighted-L2} by adding a 
weighting factor $\alpha_i\in[0,1]$, which is defined as the normalized \ti{inverse class frequency} (IF):
\begin{large}
\begin{equation}
\alpha_i = \frac{IF_i}{\sum_iIF_i}
\end{equation}
\end{large}
\begin{large}
\begin{equation}
IF_i = \frac{N}{N_i}
\end{equation}
\end{large}
% The final loss is the \ti{weighted-L2 loss}:
\begin{large}
\begin{equation}
\text{weighted-L2}(p,y)=\sqrt{\sum_{i=1}^{4}\alpha_i(p_i-y_i)^2}
\end{equation}
\end{large}
where $N$ is the number of all samples, $N_i$ is the number of samples of class $i$, $IF_i$ is the inverse class frequency. Those majority classes usually have high frequencies and thus get small $\alpha_i$ while minor classes get larger $\alpha_i$, consequently the training speed of the imbalanced data are \ti{rebalanced}.

\subsection{Training \model}
The training process of \model is presented in Algorithm 1. TDN is first pre-trained (Line 6) before the co-training process of TFN and TDN. In every batch, we first obtain the predictions of TDN and TFN via the feedforward network (Line 10-11), then we generate pseudo-labels for unlabeled grids using DLG and obtain the quality score for every pseudo-label using LQD (Line 12-13). Based on these, the the supervised and unsupervised losses are calculated respectively, then we use gradient decent to update the parameters of \model (Line 15-18). This process is repeated until convergence.
\begin{algorithm}[ht]
\caption{Training \model}
\begin{algorithmic}[1]
% $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
\REQUIRE A set of historical turbulence feature sequence $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$.\\
% \ENSURE Trained TFN$(\mc{\theta})$
\ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
\STATE $\text{I}_s=\{\text{mask unlabled grids, keep labeled}\}$.
\STATE $\text{I}_u=\{\text{mask labled grids, keep unlabeled}\}$.
\STATE $\text{T} = \{n+1,...,n+p\}$, the forecasting time stamps.
\STATE Let $\left\|\cdot \right\|_{weighted}$ denote \tb{weighted-L2}.
\STATE Let $\circ$ denote the \tb{Hadamard product}.
\STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
\WHILE{not converge}
% \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
\STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
\FOR {$({X}_h^b,{X}_f^b,{Y}^b) \in \mc{B}$}
\STATE ${P}^{b}_{\sss TFN}=\mc{F}({X}_h^b,{X}_f^b;\theta_{\sss TFN})$;
\STATE ${P}^{b}_{\sss TDN}=\mc{F}({X}_f^b;\theta_{\sss TDN})$;
\STATE Generate pseudo-label $\hat{{Y}}^{b}$ using ${P}^{b}_{\sss TFN},{P}^{b}_{\sss TDN}$ by equation (14)-(17);
\STATE Calculate label quality score $\text{S}^b$ by equation (18)-(19);
\ENDFOR
\STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}({P}^{b,t}_{\sss TFN},{Y}^{b,t}) \right )$
% \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|\right )$
\STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| {P}^{b,t}_{\sss TFN}-\hat{{Y}}^{b,t} \right \|_{weighted} \right )$
\STATE $\mc{L}=\mc{L}_s+\lambda\mc{L}_u$
\STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
\ENDWHILE
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[ht]
% \caption{Training \model}
% \begin{algorithmic}[1]
% % $\mc{X}_h =\{ (X_1,X_2,..., X_n)\}$
% \REQUIRE A set of historical turbulence feature sequence $\mc{X}_h =\{ (X_1,..., X_n)\}$, 
% % real turbulence feature sequence set $\mc{X}_r=\{(X_{n+1},..., X_{n+p})\}$, 
% forecasted turbulence feature sequence set $\mc{X}_f =\{(X'_{n+1},..., X'_{n+p})\}$, ground truth turbulence condition sequence set $\mc{Y} =\{(Y_{n+1},..., Y_{n+p})\}$.\\
% % \ENSURE Trained TFN$(\mc{\theta})$
% \ENSURE $\mc{F}(;\theta_{\sss TFN})$: parameters of trained TFN.
% \STATE Pre-train $\mc{F}(;\theta_{\sss TDN})$ based on ($\mc{X}_f$, $\mc{Y}$).
% \STATE $\text{I}_s=\{\text{mask unlabled grids}\}$
% \STATE $\text{I}_u=\{\text{mask labled grids}\}$
% \STATE $\text{T} = \{n+1,...,n+p\}$, the forecasting time stamps.
% \WHILE{not converge}
% % \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_r,\mc{X}_f,\mc{Y}$);
% \STATE sample a batch $\mc{B}$ from ($\mc{X}_h,\mc{X}_f,\mc{Y}$);
% % \FOR {$(\mc{X}_h^b,\mc{X}_r^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% \FOR {$(\mc{X}_h^b,\mc{X}_f^b,\mc{Y}^b) \in \mc{B}$}
% \STATE $\mc{P}^{b}_{\sss TFN}=\mc{F}(\mc{X}_h^b,\mc{X}_f^b;\theta_{\sss TFN})$;
% \STATE $\mc{P}^{b}_{\sss TDN}=\mc{F}(\mc{X}_f^b;\theta_{\sss TDN})$;
% \STATE Generate pseudo-label $\hat{\mc{Y}}^{b}$ using $\mc{P}^{b}_{\sss TFN},\mc{P}^{b}_{\sss TDN}$ by equation (9)-(11);
% \STATE Calculate label quality score $\mc{S}^b$ by equation (12);
% \ENDFOR
% \STATE $\mc{L}_s = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_s\circ \text{FC}(\mc{P}^{b,t}_{\sss TFN},\mc{Y}^{b,t}) \right )$
% \STATE $\mc{L}_u = \mathlarger{\frac{1}{|\mc{B}||\text{T}|}}\left ( \mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \text{T}} \text{I}_u\circ \text{S}^{b,t}\circ \left\| \mc{P}^{b,t}_{\sss TFN}-\hat{\mc{Y}}^{b,t} \right \|\right )$
% % \STATE For each $t\in \mc{T}$, sample $N_c$ unlabeled grids as central grids $\mc{C}_t$, for each $c\in \mc{C}_t$, sample $N_a$ adjacent grids as $\mc{A}_c$. 
% % \STATE $\mc{L}_r = \mathlarger{\frac{1}{|\mc{B}||\mc{T}|N_cN_a}} \left (\mathlarger\sum\limits_{b\in \mc{B}}\mathlarger\sum\limits_{t\in \mc{T}}\mathlarger\sum\limits_{c\in \mc{C}_t}\mathlarger\sum\limits_{a\in \mc{A}_c}\left \| \mc{P}^{b,t,c}_{\sss TFN}-\mc{P}^{b,t,a}_{\sss TFN} \right \|\right )$
% \STATE $\mc{L}=\mc{L}_s+\mc{L}_u$
% \STATE Compute the gradients with respect to $\mc{L}$ by backpropagation and update $\theta_{\sss TFN}$, $\theta_{\sss TDN}$ using gradient decent.
% \ENDWHILE
% \STATE$\circ$ denotes the \tb{Hadamard product}.
% \end{algorithmic}
% \end{algorithm}
